Testing learning-enabled cyber-physical systems with Large-Language Models: A Formal Approach

The integration of machine learning (ML) into cyber-physical systems (CPS) offers significant benefits, including enhanced efficiency, predictive capabilities, real-time responsiveness, and the enabling of autonomous operations. This convergence has accelerated the development and deployment of a range of real-world applications, such as autonomous vehicles, delivery drones, service robots, and telemedicine procedures. However, the software development life cycle (SDLC) for AI-infused CPS diverges significantly from traditional approaches, featuring data and learning as two critical components. Existing verification and validation techniques are often inadequate for these new paradigms. In this study, we pinpoint the main challenges in ensuring formal safety for learningenabled CPS.We begin by examining testing as the most pragmatic method for verification and validation, summarizing the current state-of-the-art methodologies. Recognizing the limitations in current testing approaches to provide formal safety guarantees, we propose a roadmap to transition from foundational probabilistic testing to a more rigorous approach capable of delivering formal assurance.

==> Backup.tex <==

\section{Related Work}
\label{sec:related}

We take an overview of related works in software vulnerabilities detection from three different categories: 
traditional rule-based approach, deep learning-based approach, and graph learning-based approach. 

For the traditional approach, early works on vulnerability detection are heavily reliant on human-crafted rules from domain experts. 
The work in~\cite{engler2001bugs} is the first of this kind to implement rules to identify software bugs and vulnerabilities automatically. 
Following that, many static analysis tools~\cite{ferschke2012flawfinder,viega2001static,kremenek2008finding, bader2019getafix, caitlin2015tricorder} 
are developed to cover some well-known security issues, all of which share the same principle 
that if the scanned code base fails to conform to the re-defined rules, 
relevant vulnerabilities could occur. 
It is infeasible to craft rules that cover all possible code vulnerabilities, 
not to mention the required efforts to cope with the ever-changing code bases.

The rapid development of machine learning, especially deep learning techniques, 
unleashes the great potential in enabling the automated learning of implicit vulnerable programming patterns. 
Many early works focus on extracting the features from lines of codes to 
facilitate vulnerability detection/prediction~\cite{chowdhury2011using,shin2010evaluating,chernis2018machine}. 
For instance, 
VulDeePecker~\cite{li2018vuldeepecker} is the first deep learning-based binary vulnerability detector, 
which slices the program into code gadgets and utilizes BiLSTM to capture the semantic relations in the data dependence within the code gadgets. 
%
Similarly, $\mu$VulDeePecker~\cite{zou2019mu} uses both BiLSTM and code attentions to capture more ``localized'' information within a code statement, 
and control dependence among method calls. 
%
LIN \textit{et al.}~\cite{lin} designs a framework that uses data sources of different types for learning unified high-level representations of code snippets. 
It also uses BiLSTM as the core component of the learning process. 
%
DeepBugs~\cite{pradel2018deepbugs} uses a feedforward network as the classifier for name-based bug detection, 
which reasons about names based on semantic representations. 
However, only the natural code sequences are considered in these works, 
and the intra-program flow logic and dependency information are omitted. 


Neural networks on graphs have drawn increasing attention in recent years, 
which focus on learning the model based on graph-structured input~\cite{li2015gated,kipf2016semi,zhang2021gps}. 
Researchers have put efforts into exploring the feasibility of using code graph representations such as 
Abstract Syntax Trees (AST), Program Dependency Graphs (PDG), and Control Flow Graphs (CFG) for vulnerability detection tasks. 
The work in~\cite{allamanis2018learning} first presents how to construct graphs from source code using AST and additional control and data flows, 
and then uses Gated Graph Neural Networks (GGNN) to detect variable misuse bugs. 
Afterwards, Devign~\cite{devign} starts to apply GNN on CPG. It extracts AST, 
program control and data dependency from CPG to create the joint graph as the composite code representation, 
from which a GGNN is designed to learn the graph-level embeddings for the downstream vulnerability detection task. 
%
FUNDED~\cite{funded} integrates data and control flow into the AST 
as the code graph representation and starts to distinguish multiple code relationships when training the GGNN, 
which is achieved by representing the input program as multiple relation graphs. 
%
DeepWukong~\cite{deepwukong} combines the CFG and PDG to generate a refined subgraph called XFG for the program, 
and adopts three different GNNs to test the performance for bug prediction. 
Existing research mainly relies on adopting homogeneous graph learning techniques, 
from which types of nodes and edges are discarded, making it infeasible to represent heterogeneous structures. 
However, we argue that the graph representations of codes convey rich semantic and logical information reflected 
in a variety of node/edge types and are intrinsic to the characteristics of heterogeneous graphs~\cite{wang2022survey}. 
This motivates us to conduct this pioneering study of heterogeneous graph learning which is shown later to improve over these state-of-the-art.


\section{Preliminary}
\label{sec:pre}

\begin{figure*}[t!]
\centering
\includegraphics[width=0.85\textwidth]{figs/cpg.png}
\caption{Sample code and corresponding generated CPG.}
\label{fig:cpg}
\end{figure*}


\subsection{Heterogeneous Graph}
\label{sec:hg}


In this section, we provide a formal definition of the heterogeneous graph~\cite{dong2017metapath2vec}. 
A heterogeneous graph $\mathcal{G = (V, E}, \mathcal{T}_v, \mathcal{T}_e)$ consists of 
a set of nodes $\mathcal{V}$ with multiple node types $\mathcal{T}_v$ and a set of edges $\mathcal{E}$ with multiple edge types $\mathcal{T}_e$. 
%
To describe the types of nodes and edges, we define two mapping functions: $ \tau : \mathcal{V} \rightarrow \mathcal{T}_v$ for the node types, 
and $ \phi : \mathcal{E} \rightarrow \mathcal{T}_e$ for the edge types. $\mathcal{X \in R^{N \times D}}$ represents the initial node feature matrix, 
where $\mathcal{N}$ is the number of nodes and $\mathcal{D}$ is the dimensionality of the feature vector. 
Finally, we define the Readout function $f : \mathcal{G} \rightarrow \mathcal{R}^{1 \times n}$, 
which summarizes the node and edge features and generates a low-dimensional graph-level embedding with $n$ dimensions.



\subsection{Code Property Graph}
The Code Property Graph (CPG) is a data structure representing source code, 
program structure, and execution logic in a unified graph-based representation~\cite{yamaguchi2014modeling}. 
It encapsulates the entire program in a single graph that consists of nodes and edges with multiple types, 
in which each node represents an entity, such as a function/method, a variable, or a class, 
and each edge represents a relationship between the entities. 
CPGs provide a comprehensive view of the program and enable the analysis of code properties 
and behaviors with the help of control flow, data flow, and intra-program dependence.

\textbf{Fig.~\ref{fig:cpg}} shows a toy example of CPG and its corresponding code snippet. 
For simplicity, we keep primary control/data flows, program dependence and execution steps for demonstrative purposes, 
while the specific AST edge types are not shown. 
The $\epsilon$ in \textbf{Fig.~\ref{fig:cpg}B} describes the control flow without any condition predicates when executing the program. 
The program steps over to the condition predicate statement and 
jumps to different statements based on \textit{true} or \textit{false} conditions (line 6 and 10 in \textbf{Fig.~\ref{fig:cpg}A)}. 
The blue edge represents both data and control dependence in the program. 
For instance, $D_{VAR1}$ shows the data dependence of variable \textit{VAR1} initially declared at line 3, 
and $C_{true}$ indicates that the variable declaration statement at line 6 is dependent on the condition predicate at line 5. 
The green edge is the simplified relationships in the abstract syntax tree (AST), 
where the inner nodes represent \textit{operators} (e.g., addition, assignment) 
and leaf nodes as \textit{operands} (e.g., variable identifier, constants). 
The full descriptions of node types and edge types in the CPG can be found in Table~\ref{tab:node} and Table~\ref{tab:edge}.


\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\textwidth]{figs/simple_graph_construction.png}
\caption{Graph Construction}
\label{fig:graph-cons}
\end{figure*}


\subsection{Heterogeneous Graph Transformer}
\label{sec:hgt}

To capture the complex interactions between various types of entities in heterogeneous graphs, 
Hu \textit{et al.} proposed Heterogeneous Graph Transformer (HGT)~\cite{hu2020heterogeneous}, 
which introduces the transformer into the graph neural network to better incorporate the heterogeneous nature of the graph structure.
% \textcolor{red}{HGT also has the ability to extract hidden features from graph data.}
% For CPG, HGT is able to fully learn the features contained in it, which enables to improve the robustness of the model and perform deeper code semantic analysis.

In HGT,
a triplet $<\tau(s), \phi(e) ,\tau(t)>$ can be used to denote the relationships among 
source node ($s$), directed edge ($e$), and target node ($t$).
The function $\tau(\cdot)$ is node type mapping, which outputs the type of input node. 
Similarly, function $\phi(\cdot)$ denotes the edge type mapping, which outputs the type of input edge. 
%
This triplet and the original node embedding for the source and target nodes are the input for HGT. 
The embedding of nodes is updated through multiple iterations, each of which includes three steps:
\textit{1)} Attention calculation (Section~\ref{sec:attention});
\textit{2)} Message calculation (Section~\ref{sec:message});
and \textit{3)} Aggregation of attention and message (Section~\ref{sec:aggregate}). 
We will detail our adaptation of HGT in Section~\ref{sec:method-hgt-multi-task}.



\section{Heterogeneous Graph Learning}
\label{sec:method}

In our proposed heterogeneous graph learning procedure, we have the following two main steps. 
The first step is Graph Construction (shown in \textbf{Fig.~\ref{fig:graph-cons}}). 
We analyze all the source code and generate the initial CPG
(\textbf{Fig.~\ref{fig:graph-cons}A} \& \textbf{Fig.~\ref{fig:graph-cons}B}). 
%
As we focus on method-level vulnerability analysis in this pioneering study, 
we extract method-level CPGs from the initial CPG  (\textbf{Fig.~\ref{fig:graph-cons}C}).
%
Meanwhile, symbolization is also performed on method-level CPGs to 
reduce the noise introduced by personalized function/variable naming conventions (\textbf{Fig.~\ref{fig:graph-cons}D}).
%
We then perform the embedding method for each node within 
the method-level CPGs for the next step (\textbf{Fig.~\ref{fig:graph-cons}E}).


The second step is our adaptation of HGT - Dual-Supervisors HGT Learning (shown in \textbf{Fig.~\ref{fig:hgt-multi}}). 
In Dual-Supervisors  HGT learning, 
we use initial node features as the input of HGT to learn and extract the graph-level information. 
\textcolor{red}{CPG contains heterogeneous features, and HGT, as a heterogeneous transformer network, can effectively extract and learn these features to improve the robustness of the model.}
We then leverage dual-supervisors learning for both vulnerability prediction and \textcolor{red}{code comment} generation. 
We introduce the \textcolor{red}{code comment} as the second supervisor to align the latent features 
learned from the HGT with the underlying semantic meaning through the back-propagation process.



\subsection{Graph Construction}
\label{sec:method-graph}


We first analyze all the source code files 
and generate the initial corresponding Code Property Graphs (CPGs). 
In our case, all the related files (\textit{e.g.} source code files and dependency library files) 
are within the same directory. By inputting this directory to an open source 
code parser \textit{Joern}\footnote{https://github.com/joernio/joern}, 
these source code files are then iterated automatically to generate the corresponding CPG.



\begin{algorithm}[h!]
\caption{Generating Method-level Code Property Graph}
\label{alg:method-cpg}
\begin{algorithmic}[1]

\Require Source code root directory \textit{S}, \textit{Joern} parser \textit{J}
\OUTPUT Method-level CPGs set \textit{M}.
\State \textit{C} $\leftarrow$ $\emptyset$
\For{each leaf directory \textit{l} $\in$ dir(\textit{S})}
    \State  generate CPG \textit{c} through \textit{J}(\textit{l}), and add to set \textit{C}
\EndFor
\State \textit{M} $\leftarrow$ $\emptyset$
\For{each \textit{c} $\in$ \textit{C}}
    \State  \textit{N} $\leftarrow$all \textit{method} type nodes within \textit{c}
    \For{each \textit{n} $\in$ \textit{N}}
        \State start at \textit{n}, perform DFS forward traverse  
        \State start at \textit{n}, perform DFS backward traverse
        \State generate method-level CPG \textit{m} for method \textit{n}
        \State add \textit{m} to set \textit{M}
    \EndFor
\EndFor

\end{algorithmic}
\end{algorithm}

In this paper, we concentrate on method-level vulnerability analysis, 
and Algorithm~\ref{alg:method-cpg} demonstrates how we construct the method-level CPGs. 
As indicated in the pseudo-code,
the generated CPG is denoted as $\mathit{c}$, which contains all relationships of source codes
within one leaf directory. The set of all directory-level CPGs is denoted as $\mathit{C}$. 
Instead of using original CPG $\mathit{c}$ that contains much redundant information in the graph, 
we perform forward and backward traversal to generate the method-level CPG $\mathit{m}$. 
Specifically, both traversals are based on Depth-First Search (DFS) for each \textit{Method} node within $\mathit{c}$, 
and the set of all method-level CPGs is denoted as $\mathit{M}$. Taking \textbf{Fig~\ref{fig:graph-cons}C} as an example, 
node \textit{3} is a method node, from which we traverse forward through nodes \textit{6,7,8,11,13,14,15}, 
while traversing backward through the node \textit{1}. 
Thus all the nodes be traversed are \textit{1,3,6,7,8,11,13,14,15} including itself.
Thus, the corresponding method-level CPG (Method\_CPG) could be generated by slicing this traversed set out of the original CPG.

In each CPG (\textbf{Fig~\ref{fig:graph-cons}B}), 
we construct the heterogeneous graph by mapping the original entities (e.g., Method name) and relationships (e.g., method call) to
different types of nodes (e.g., \textit{METHOD}) and edges (e.g., \textit{CALL}).
%
For a full list of nodes and edges we generated for CPG, 
please refer to Table~\ref{tab:node} and Table~\ref{tab:edge}.


% symbolization
Meanwhile, 
to alleviate the noise introduced by personalized naming conventions 
for functions and variables and better preserve the original code semantics~\cite{deepwukong}, 
we then perform symbolization on method-level CPGs (shown in \textbf{Fig~\ref{fig:graph-cons}D}). Following that,
different function and variable names defined by users will be unified to \textit{METHOD`N'(~)} and \textit{VAR`N'}, where $N\in\mathbb{Z}^{+}$. 
For example, the function names \textit{readData(~)} and \textit{writeData(~)} 
and variable names \textit{x} and \textit{y} 
will be mapped to \textit{METHOD1(~)}, \textit{METHOD2(~)}, \textit{VAR1}, and \textit{VAR2}, respectively. 
The actual numbers $N$ used in the symbolization may vary.
% embedding
As shown in \textbf{Fig~\ref{fig:graph-cons}E},
we then perform Doc2Vec embedding~\cite{le2014distributed} for each node within the method-level CPGs. 
This embedding serves as the initial node feature and will be refined during the Dual-Supervisors HGT learning.



\subsection{Dual-Supervisors HGT Learning}
\label{sec:method-hgt-multi-task}


\begin{figure*}[h!]
\centering
\includegraphics[width=0.9\textwidth]{figs/hgt_multitask.png}
\caption{\textit{DSHGT} Learning}
\label{fig:hgt-multi}
\end{figure*}


%An example of extracting CPG information through HGT 
The overall architecture of the Dual-Supervisors HGT (\textit{DSHGT}) is shown in \textbf{Fig~\ref{fig:hgt-multi}}.
For each target node in a given CPG, we consider all its connected neighbors as source nodes, 
and for each source node/target node pair we define $<\tau(s),\phi(e),\tau(t)>$ triplet as the relationship of this pair (shown in \textbf{Fig~\ref{fig:hgt-multi}A}). 
For each triplet, we then calculate the attention score between the source node and the target node (shown in \textbf{Fig~\ref{fig:hgt-multi}B}), 
calculate the messaging passing score of each source node (shown in \textbf{Fig~\ref{fig:hgt-multi}C}), 
and aggregate the information from the above two steps and update the target node embedding (shown in \textbf{Fig~\ref{fig:hgt-multi}D}). 
% \textcolor{red}{HGT is able to learn these potential features better and more accurately.}
To improve the robustness of the learned features (aggregated target node embedding), 
we use the existing \textcolor{red}{code comment} for each method as the additional supervisor in the multi-task learning (shown in \textbf{Fig~\ref{fig:hgt-multi}E}). 
We will walk through each step in more details below.


Note, we use $H^{\alpha}[\beta]$ to denote node $\beta$'s embedding in the $\alpha$-th layer, 
and $H^{\alpha-1}[\beta]$ to denote node $\beta$'s embedding in the $(\alpha-1)$-th layer, 
through the whole section.


\subsubsection{Constructing \textit{DSHGT} Input Triplet (Fig~\ref{fig:hgt-multi}A)} 

For each method CPG, we iteratively walk through the CPG using the depth-first search algorithm and construct the triplet from the root level all the way to the leaf nodes. 
For instance, when we walk to the node of \{11\} (\textit{i.e.} node $t$) in \textbf{Fig~\ref{fig:hgt-multi}A}, 
we treat the node as the current target node. 
We found its neighbor nodes are \{8\}, \{15\}, \{14\} and \{13\} (\textit{i.e.} node $s_1$, $s_2$, $s_3$ and $s_4$, respectively). 
Then we construct the following triplets 
$<\tau(s_1), \phi(e) ,\tau(t)>$, 
$<\tau(s_2), \phi(e) ,\tau(t)>$, 
$<\tau(s_3), \phi(e) ,\tau(t)>$ 
and 
$<\tau(s_4), \phi(e) ,\tau(t)>$.
We then feed them all to the \textit{DSHGT}. 
Note, to simplify the figure, we only present the embedding 
for node $t$, $s_1$ and $s_2$ in \textbf{Fig~\ref{fig:hgt-multi}}.


\subsubsection{Heterogeneous Attention Calculation (Fig~\ref{fig:hgt-multi}B)}
\label{sec:attention}

Firstly, we calculate the attention between $s_1$ and $t$, where $s_1$ is one of the neighbor nodes of $t$. 
The calculation involves five equations (Eq.~\ref{eq:q-linear} to Eq.~\ref{eq:attention}).


\begin{equation}
\label{eq:q-linear}
    Q^i(t) =   H^{(l-1)}[t] \cdot Q{\text{-}}Linear^i_{\tau(t)}
\end{equation}
where the dimension of $H^{(l-1)}[t]$ (\textit{i.e.} the embedding of $t$) is $R^{1 \times d}$, 
the dimension of $Q{\text{-}}Linear^i_{\tau(t)}$ is $R^{d \times \frac{d}{h}}$, 
 $i$ ($i \in [1,h]$) represent the $i$-th head of attention, 
and the dimension of $Q^i(t)$ is $R^{1 \times \frac{d}{h}}$.
%
We project $H^{(l-1)}[t]$ to $Q^i(t)$ through $Q{\text{-}}Linear^i_{\tau(t)}$ (\textit{i.e.} the query matrix), 
and each $\tau(\cdot)$ has 
its own matrix $Q{\text{-}}Linear^i_{\tau(t)}$ on the $i$-th head.



\begin{equation}
\label{eq:k-linear}
 K^i(s_1) =  H^{(l-1)}[s_1] \cdot K{\text{-}}Linear^i_{\tau(s_1)}
 \end{equation}

In Eq.~\ref{eq:k-linear}, the dimension of $H^{(l-1)}[s_1]$ (\textit{i.e.} the embedding of $s_1$) is $R^{1 \times d}$, 
the dimension of $K{\text{-}}Linear^i_{\tau(s_1)}$ is $R^{d \times \frac{d}{h}}$, 
where $i$ ($i \in [1,h]$) represent the $i$-th head of attention, 
and the dimension of $K^i(s_1)$ is $R^{1 \times \frac{d}{h}}$.
%
We project $H^{(l-1)}[s_1]$ to $K^i(t)$ through $K{\text{-}}Linear^i_{\tau(s_1)}$ (\textit{i.e.} the key matrix), 
and each $\tau(\cdot)$ has 
its own matrix $K{\text{-}}Linear^i_{\tau(s_1)}$ on the $i$-th head.


\begin{equation}
\label{eq:i-attention}
ATT{\text -}head^i(s_1,e,t)=(K^i(s_1) \times W^{ATT}_{\phi(e)} \times Q^i(t)^T) \times \frac{\mu_{<\tau(s_1),\phi(e),\tau(t)>}}{\sqrt{d}} 
\end{equation}

Eq.~\ref{eq:i-attention} is for calculating the attention value of the $i$-th head from $s_1$ to $t$.
The $W^{ATT}_{\phi(e)} \in R^{\frac{d}{h} \times \frac{d}{h}}$ stands for a learnable parameter matrix for edge type $\phi(e)$,
which represents the learnable semantic information for each edge type. 
%
The $(K^i(s_1) \times W^{ATT}_{\phi(e)} \times Q^i(t)^T)$ is the original attention value of the $i$-th head. 
The dimension of it is $R^{1 \times 1}$ 
(\textit{i.e.} $R^{1 \times \frac{d}{h}} \times R^{\frac{d}{h} \times \frac{d}{h}} \times R^{\frac{d}{h} \times 1} \rightarrow R^{1 \times 1}$). 
%
The $\mu$ is a matrix related with the triplet $<\tau(s_1),\phi(e),\tau(t)>$, 
which acts as a scaling factor for this triplet relationship.
Its dimension is $R^{A \times E \times A}$, 
where $A = |\tau(\cdot)|$ and $E = |\phi(\cdot)|$. 
%
It is worth noting that, the magnitude of $K$ and $Q$ dot product increases significantly
and will lead \textit{Softmax} function to small gradient values.
Thus, we divide the original value by $\sqrt{d}$ to
maintain the gradient values after \textit{Softmax}, 
which could help the training. 


\begin{equation}
\label{eq:1-attention}
\textbf{Attention}_{DSHGT}(s_1, e ,t) = \mathop{\parallel}\limits_{i \in[1, h]} ATT{\text -}head^i(s_1, e, t)
\end{equation}

Eq.~\ref{eq:1-attention} is for calculating the attention value from $s_1$ to $t$. 
The $h$ heads attention values from Eq.~\ref{eq:i-attention} will be concatenated 
together to a vector with $R^{h \times 1}$ dimensions.
Note the attention calculation will be the same 
for all the triplets, $<\tau(s_2), \phi(e) ,\tau(t)>$, $<\tau(s_3), \phi(e) ,\tau(t)>$, \textit{etc.}

To yield the final attention value for each head, we gather attention matrices 
from all neighbors of $N(t)$ and conduct \textit{Softmax} as shown in Eq.~\ref{eq:attention}. 

\begin{equation}
\label{eq:attention}
\textbf{Attention}_{DSHGT}(s, e ,t) = \mathop{Softmax}\limits_{\forall{s \in N(t)}} \left(   \textbf{Attention}_{DSHGT}(s, e ,t)   \right)
\end{equation}

\subsubsection{Heterogeneous Message Calculation (Fig~\ref{fig:hgt-multi}C)}
\label{sec:message}

Secondly, we shows how to calculate the message from $s_1$ to $t$, 
which involves three equations (Eq.~\ref{eq:v-linear} to Eq.~\ref{eq:message}).

\begin{equation}
\label{eq:v-linear}
V^i(s_1) = H^{(l-1)}[s_1] \cdot V{\text{-}}Linear^i_{\tau(s_1)}
\end{equation}

In Eq.~\ref{eq:v-linear}, 
the dimension of $H^{(l-1)}[s_1]$ is $R^{1 \times d}$, 
the dimension of $V{\text{-}}Linear^i_{\tau(s_1)}$ is $R^{d \times \frac{d}{h}}$, 
where $i$ ($i \in [1,h]$) represent the $i$-th head of message, 
and the dimension of $V^i(s_1)$ is $R^{1 \times \frac{d}{h}}$.
%
We project $H^{(l-1)}[s_1]$ to $V^i(s_1)$ through $V{\text{-}}Linear^i_{\tau(s_1)}$ (\textit{i.e.} the value dimension), 
and each $\tau(\cdot)$ has 
its own parameter $V{\text{-}}Linear^i_{\tau(s_1)}$ on the $i$-th head.

\begin{equation}
\label{eq:i-message}
    MSG{\text -}head^i(s_1, e, t) = V^i(s_1) \times W^{MSG}_{\phi(e)} 
\end{equation}



Eq.~\ref{eq:i-message} calculates the message value of the $i$-th head from $s_1$ to $t$.
The $W^{MSG}_{\phi(e)} \in R^{\frac{d}{h} \times \frac{d}{h}}$ stands for a learnable parameter matrix for edge type $\phi(e)$, 
and each $\phi(\cdot)$ has its own $W^{MSG}_{\phi(e)}$ matrix. 
%
The dimension of $MSG{\text -}head^i(s_1, e, t)$  is $R^{1 \times \frac{d}{h}}$ 
(\textit{i.e.} $R^{1 \times \frac{d}{h}} \times R^{\frac{d}{h} \times \frac{d}{h}} \rightarrow R^{1 \times \frac{d}{h}} $). 



\begin{equation}
\label{eq:message}
    \textbf{Message}_{DSHGT}(s_1, e ,t) = \mathop{\parallel}\limits_{i \in[1, h]} MSG{\text -}head^i(s_1, e, t)
\end{equation}

The message value from $s_1$ to $t$ is calculated in Eq.~\ref{eq:message}, 
in which the $h$ heads message values from Eq.~\ref{eq:i-message} will be concatenated 
together to a matrix with $R^{h \times \frac{d}{h}}$ dimensions.
Note the message calculation will be the same 
for all the triplets, $<\tau(s_2), \phi(e) ,\tau(t)>$, $<\tau(s_3), \phi(e) ,\tau(t)>$, \textit{etc.}



\subsubsection{Heterogeneous Node Embedding Aggregation(Fig~\ref{fig:hgt-multi}D)}
\label{sec:aggregate}

Thirdly, we calculate the aggregation of attention and message from $s_1$ to $t$. 

\begin{equation}
\label{eq:aggregate-1}
    \tilde{H}^l[t_{s_1}] =  \textbf{Attention}_{DSHGT}(s_1, e ,t) \otimes \textbf{Message}_{DSHGT}(s_1, e ,t)
\end{equation}


The weighted message from $s_1$ is shown in Eq.~\ref{eq:aggregate-1},
where $\otimes$ is element-wise multiplication. The dimension of $\textbf{Attention}_{DSHGT}(s_1, e ,t))$ is $R^{h \times 1}$, 
and the dimension of $\textbf{Message}_{DSHGT}(s_1, e ,t)$ is $R^{h \times \frac{d}{h}}$. 
Note the weighted message calculation will be the same for all the triplets.

After calculating the weighted message for all neighbors of $N(t)$, 
we could update the target node $t$ embedding based on messages from its neighbors. 

\begin{equation}
\label{eq:aggregate-2}
    \tilde{H}^l[t] = \mathop{\oplus}\limits_{\forall{s \in N(t)}} \tilde{H}^l[t_{s}]
\end{equation}


We then reshape the vector to $\tilde{H}^l[t] \in R^{1 \times d}$.


\begin{equation}
\label{eq:aggregate-residual}
    H^l[t] = \alpha\left( \tilde{H}^l[t] \cdot A{\text -}Linear_{\tau(t)} \right) + H^{l-1}[t] 
\end{equation}

In Eq.~\ref{eq:aggregate-residual},
the $\tilde{H}^l[t]$ stands for the node $t$ embedding for current layer, 
the $H^{l-1}[t]$ stands for the node $t$ embedding from previous layer, 
the $\alpha$ is the activation function (\textit{i.e.} ReLU). 
We project $\tilde{H}^l[t]$ through $A{\text{-}}Linear_{\tau(t)} \in R^{d \times d}$. 
Note each $\tau(\cdot)$ has its own parameter in $A{\text{-}}Linear_{\tau(t)}$. 
The projection (\textit{i.e.} $A{\text -}Linear_{\tau(t)}\left(\tilde{H}^l[t]\right)$) will then 
go through the activation function before adding up the node $t$ embedding from the previous layer as residual, 
and yield the final node $t$ embedding for the current layer.
%
In one iteration, we update all the nodes' embedding within the heterogeneous graph following the same procedure.
We iterate this calculation for every nodes within the method-level CPG for $L$ layers. 
The $L$-th layer output $H^L[t]$ (\textbf{Fig~\ref{fig:hgt-multi}D}) will be used for downstream tasks.



\subsubsection{Dual-Supervisors Learning (Fig~\ref{fig:hgt-multi}E)}


The \textit{DSHGT} node embedding procedure will go through $L$ times (\textit{i.e.} $L$ layers of \textit{DSHGT}),
and each layer will use the previous layer's embedding as input 
(the initial layer's input is based on the CPG embedding, 
details in Section~\ref{sec:method-graph}).
In our experiments, we perform empirical study and set $L = 3$ (details analyzed in Section~\ref{sec:rq3}).
As the output form \textit{DSHGT} (\textit{i.e.} $H^L[t]$) is node-based embedding, 
we construct a \textit{Readout} layer for graph-level embedding output:

\begin{equation}
\label{readout}
    z^{\mathcal{G}}=M E A N\left(M L P\left(\mathcal{X} \oplus H^L\right)\right)
\end{equation}


Instead of directly taking out the embeddings, 
we concatenate them with the initial node embedding, pass through a shallow multi-layer perceptron (MLP),
and follow with a row-wise \textit{MEAN} operation.
%
$\mathcal{X}$ is defined in Section~\ref{sec:hg}, which represents the initial node embedding. 

This output then goes through a dual-supervisors structure(\textit{i.e.} MLP and Decoder) 
for multi-task purposes (\textbf{Fig~\ref{fig:hgt-multi}E}).
%
For detecting vulnerabilities within the source code (\textbf{Fig~\ref{fig:hgt-multi}E(\textit{b})}), 
we use 1 layer MLP for \textbf{0/1} classification, 
where \textbf{0} stands for no vulnerability while \textbf{1} means the source code segment contains vulnerabilities.
\textcolor{red}{We only test whether the code snippets contain vulnerabilities, and do not classify them into a specific type of CWE.}
On the other hand, We consider the graph-level embedding as an \textit{Encoder} for the source code 
and design the corresponding \textit{Decoder} (1-layer LSTM) to summarize 
the corresponding source \textcolor{red}{code comments} sequence-to-sequence (\textbf{Fig~\ref{fig:hgt-multi}E(\textit{c})}). 
Then we compare the generated \textcolor{red}{code comments} with \textcolor{red}{comments} within source code (\textit{i.e.} the ground truth) 
and yield cross entropy loss for multi-tasks. 
%
To leverage the \textit{loss} from the two supervisors, 
we implement the following equation for \textit{loss} fusion: 

\begin{equation}
\label{eq:multi-task-weight}
    loss = (1-\lambda) \times loss_{main} + \lambda \times loss_{sup}
\end{equation}

In Eq.~\ref{eq:multi-task-weight}, 
$loss_{main}$ is the \textit{loss} of $0/1$ classification and $loss_{sup}$ is the \textit{loss} of \textcolor{red}{code comments} prediction. 
The $\lambda$ is the parameter for adjusting the weight of $loss_{sup}$ in $loss$. 



\section{Experiment}
\label{sec:exp}

We evaluate the performance of our framework on different datasets 
against a number of state-of-the-art graph-based or traditional vulnerability detection models. 
We aim to answer the following research questions.


\begin{itemize}
\setlength{\itemindent}{-2.5em}
    \item[] \textbf{RQ1}: How well our proposed framework performs compared with other baselines in public C/C++ vulnerability datasets?
    \item[] \textbf{RQ2}: Can the framework achieve a consistently higher vulnerability detection capability when applied to other programming languages? 
    \item[] \textbf{RQ3}: How to balance the contribution from the two supervisors 
    (i.e., vulnerability and \textcolor{red}{code comment} oracles) to improve the performance?
    \item[] \textbf{RQ4}: How much can the CPG input representation and HGT backbone improve the performance?
    \item[] \textbf{RQ5}: How effective is our proposed method when applied to detect vulnerabilities in real-world open-source projects? 
\end{itemize}




\subsection{Experimental Setup}
We describe the experimental setup in this section, 
including the environment, baselines, evaluation metrics, and the datasets preparation.
\textcolor{red}{The parameters information of models are shown in Table \ref{tab:model}.}

\begin{table}[h!]
\centering
\caption{\textcolor{red}{\textcolor{red}{Information of models parameters}}}
\label{tab:model}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|c|}
\hline
Model Information & HGT     & Decoder & MLP    & Total   \\ \hline
Number of Parameters  & 5,091,894 & 46,280   & 12,456  & 5,150,720 \\ \hline
Size              & 5.09 MB & 0.05 MB & 0.01MB & 5.15MB  \\ \hline
\end{tabular}
}
\end{table}




\subsubsection{Environment}
We implemented our heterogeneous graph-based vulnerability detection model using Python v3.7 and Pytorch v1.11.0. 
As mentioned in Section~\ref{sec:method-graph}, 
we leveraged \textit{Joern} to 
generate the initial CPG of different programming languages. 
We trained and tested our model on a computer with an 8-core 3.8 GHz Intel Xeon CPU and an NVIDIA 3080Ti GPU. 
The hyperparameter setup could be found in Table~\ref{tab:hyper}.


\subsubsection{Baselines}
We compared our \tool~with the following state-of-the-art baselines and reported the comparison statistics.

\begin{itemize}
\setlength{\itemindent}{-2.5em}

    \item[] \textbf{LIN \textit{et al.}}~\cite{lin} designs a framework that uses data sources of 
    different types for learning unified high-level representations of code snippets. 
    It uses BiLSTM as the core component of the learning process.
    
    
    \item[] \textbf{DEVIGN}~\cite{devign} combines AST, program control and data 
    dependency as the joint graph to represent the composite code representation, 
    from which a gated graph neural network model is designed 
    to learn the graph-level embeddings for the vulnerability detection task.
    
    \item[] \textbf{FUNDED}~\cite{funded} integrates data and control flow into the AST as the code graph representation, 
    which is then used as the input for the gated graph neural network (GGNN) to train the vulnerability detection model. 
    It uses Word2Vec~\cite{mikolov2013efficient} to generate the initial node embedding. 
    
    \item[] \textbf{DeepWukong}~\cite{deepwukong} is also a graph learning-based approach that 
    encodes both textual and structured information of code into code representations. 
    It is designed specifically to detect C/C++ vulnerabilities. 
    It uses Doc2Vec~\cite{le2014distributed} to generate initial node embeddings from PDG.
    % \textcolor{red}{Unlike the way \textbf{DeepWukong} constructs the dataset (based on point of intersted), we construct the dataset for each function separately. Therefore, the experiment results of \textbf{DeepWukong} in this paper are different from those of Cheng et al.}
    
\end{itemize}



Note that for all baseline models, we used the default hyperparameters as reported in the respective literature.



\subsubsection{Evaluation Metrics}

We used \textbf{Accuracy}, \textbf{Precision}, \textbf{Recall} 
and \textbf{F1} scores to evaluate the vulnerabilities detected by a model, 
which are widely used in the machine learning community to 
verify the generalization ability of a predictive model~\cite{lin2020software}.



\subsubsection{Dataset Preparation}

We used several vulnerability datasets to verify our model 
and compared the performance with baseline models. 

For \textbf{RQ1} to \textbf{RQ4}, we chose the 
\textit{Software Assurance Reference Dataset} (\textbf{SARD}), 
which is a widely used vulnerability database with 
a large set of synthetic programs~\cite{funded,deepwukong,lin2020software}. 
In \textbf{SARD}, a program is labelled as good (not vulnerable), 
bad (vulnerable) or mix (vulnerable with patched updates). 
For vulnerable programs, \textbf{SARD} describes the vulnerability and the vulnerability type 
in \textbf{CWE-ID} (\textbf{C}ommon \textbf{W}eakness \textbf{E}numeration \textbf{ID}entifier) formats. 
It also contains the human-crafted annotations in the program as supplementary information of the codes. 
We used a total of \textcolor{red}{22} categories for C/C++, Java and PHP, \textcolor{red}{of which are the 10 most common types in 2022 \textbf{CWE} Top 25 Most Dangerous Software Weaknesses\footnote{https://cwe.mitre.org/top25/archive/2022/2022\_cwe\_top25.html} and the rest 12 are most typical of other types.}
\textcolor{red}{Regarding the sample numbers of each type in \textbf{CWE} we present and explain in detail in Table \ref{tab:dataset}.}
\textcolor{red}{In each type, we selected 80\% of the sample size as the training dataset and 20\% as the test dataset.}
These categories are harvested from \textbf{SARD}, 
which is comprehensive and covers most of the vulnerability types.

For \textbf{RQ5}, we leveraged two real-world open-source projects, 
\textbf{\textit{FFmpeg}}\footnote{https://ffmpeg.org/} 
and 
\textbf{\textit{QEMU}}\footnote{https://www.qemu.org/}.
%
These two large open-source projects are written in C, involving many contributions and code commits from software developers. 
The labels of \textbf{\textit{FFmpeg}} and \textbf{\textit{QEMU}} 
are based on vulnerability-fix commits or non-vulnerability fix commits of these projects. 
The Vulnerability fix commits (VFCs) are the code commits that fix a potential vulnerability of a function/method, 
while the non-vulnerability-fix commits (non-VFCs) are commits considered less relevant to fix vulnerabilities.
The detailed statistics and descriptions of the datasets can be found in Table~\ref{tab:dataset}. 



\begin{table}[t!]
\centering
\caption{Hyperparameter setup}
\label{tab:hyper}
\scalebox{0.8}{
\begin{tabular}{c||c}
\hline
Name & \ Setup\\
\hline
\hline
Readout func (HGT) & 2 linear layers, 1 output layer   \\
Layer depth (HGT) & 3 \\
Attention head (HGT) & 4 \\
Loss function & Cross entropy loss   \\
Optimizer & Adam~\cite{kingma2014adam}\\
Learning rate & 2e-3 \\
Dropout rate & 0.5 \\
Batch size & 64\\
Epochs & 50\\
Weight initializer & Xavier~\cite{glorot2010understanding}\\

\hline
\end{tabular}
}
\end{table}




\begin{table*}[t!]
\caption{Results of the comparison with different baselines on SARD} 
\label{tab:results_25}
\scalebox{0.9}{

\begin{tabular}{|l|ll|ll|ll|ll|ll|ll|}
\hline
\multirow{3}{*}{\diagbox[]{DataSet}{Metric}{Model}} & \multicolumn{2}{l|}{\multirow{2}{*}{DEVIGN}} & \multicolumn{2}{l|}{\multirow{2}{*}{LIN et al.}} & \multicolumn{2}{l|}{\multirow{2}{*}{FUNDED}}       & \multicolumn{2}{l|}{\multirow{2}{*}{DeepWukong}} & \multicolumn{2}{l|}{\multirow{2}{*}{DSHGTnoAnno}}  & \multicolumn{2}{l|}{\multirow{2}{*}{DSHGT}}        \\
                        & \multicolumn{2}{l|}{}                        & \multicolumn{2}{l|}{}                            & \multicolumn{2}{l|}{}                              & \multicolumn{2}{l|}{}                            & \multicolumn{2}{l|}{}                              & \multicolumn{2}{l|}{}                              \\ \cline{2-13} 
                        & \multicolumn{1}{l|}{ACC}             & F1    & \multicolumn{1}{l|}{ACC}               & F1      & \multicolumn{1}{l|}{ACC}           & F1            & \multicolumn{1}{l|}{ACC}               & F1      & \multicolumn{1}{l|}{ACC}           & F1            & \multicolumn{1}{l|}{ACC}           & F1            \\ \hline
CWE-119                 & \multicolumn{1}{l|}{0.79}            & 0.81  & \multicolumn{1}{l|}{\textbf{0.85}}     & 0.78    & \multicolumn{1}{l|}{0.83}          & 0.85          & \multicolumn{1}{l|}{0.82}              & 0.84    & \multicolumn{1}{l|}{0.80}          & 0.86          & \multicolumn{1}{l|}{0.84}          & \textbf{0.87} \\ \hline
CWE-400                 & \multicolumn{1}{l|}{\textbf{0.84}}   & 0.81  & \multicolumn{1}{l|}{0.79}              & 0.76    & \multicolumn{1}{l|}{\textbf{0.84}} & 0.80          & \multicolumn{1}{l|}{\textbf{0.84}}     & 0.79    & \multicolumn{1}{l|}{0.82}          & 0.83          & \multicolumn{1}{l|}{0.83}          & \textbf{0.85} \\ \hline
CWE-404                 & \multicolumn{1}{l|}{0.84}            & 0.82  & \multicolumn{1}{l|}{0.83}              & 0.74    & \multicolumn{1}{l|}{0.81}          & 0.85          & \multicolumn{1}{l|}{0.83}              & 0.84    & \multicolumn{1}{l|}{0.83}          & 0.88          & \multicolumn{1}{l|}{\textbf{0.88}} & \textbf{0.90} \\ \hline
CWE-369                 & \multicolumn{1}{l|}{0.83}            & 0.78  & \multicolumn{1}{l|}{0.82}              & 0.80    & \multicolumn{1}{l|}{0.86}          & 0.84          & \multicolumn{1}{l|}{\textbf{0.91}}     & 0.87    & \multicolumn{1}{l|}{0.90}          & \textbf{0.91} & \multicolumn{1}{l|}{0.89}          & 0.88          \\ \hline
CWE-191                 & \multicolumn{1}{l|}{0.82}            & 0.76  & \multicolumn{1}{l|}{0.80}              & 0.73    & \multicolumn{1}{l|}{\textbf{0.87}} & 0.90          & \multicolumn{1}{l|}{0.75}              & 0.81    & \multicolumn{1}{l|}{0.81}          & 0.87          & \multicolumn{1}{l|}{0.85}          & \textbf{0.91} \\ \hline
CWE-476                 & \multicolumn{1}{l|}{0.91}            & 0.87  & \multicolumn{1}{l|}{0.89}              & 0.83    & \multicolumn{1}{l|}{0.83}          & 0.87          & \multicolumn{1}{l|}{\textbf{0.90}}     & 0.86    & \multicolumn{1}{l|}{0.85}          & 0.84          & \multicolumn{1}{l|}{0.86}          & \textbf{0.89} \\ \hline
CWE-467                 & \multicolumn{1}{l|}{0.79}            & 0.84  & \multicolumn{1}{l|}{0.87}              & 0.81    & \multicolumn{1}{l|}{0.85}          & 0.86          & \multicolumn{1}{l|}{0.88}              & 0.86    & \multicolumn{1}{l|}{0.86}          & 0.83          & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.87} \\ \hline
CWE-78                  & \multicolumn{1}{l|}{0.82}            & 0.84  & \multicolumn{1}{l|}{\textbf{0.89}}     & 0.79    & \multicolumn{1}{l|}{0.83}          & \textbf{0.86} & \multicolumn{1}{l|}{0.84}              & 0.83    & \multicolumn{1}{l|}{0.84}          & 0.86          & \multicolumn{1}{l|}{0.85}          & 0.84          \\ \hline
CWE-772                 & \multicolumn{1}{l|}{0.83}            & 0.77  & \multicolumn{1}{l|}{0.85}              & 0.81    & \multicolumn{1}{l|}{0.86}          & 0.87          & \multicolumn{1}{l|}{0.86}              & 0.83    & \multicolumn{1}{l|}{0.86}          & 0.88          & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.88} \\ \hline
CWE-190                 & \multicolumn{1}{l|}{0.86}            & 0.83  & \multicolumn{1}{l|}{0.83}              & 0.79    & \multicolumn{1}{l|}{0.86}          & 0.84          & \multicolumn{1}{l|}{0.87}              & 0.83    & \multicolumn{1}{l|}{0.85}          & 0.82          & \multicolumn{1}{l|}{\textbf{0.92}} & \textbf{0.87} \\ \hline
CWE-770                 & \multicolumn{1}{l|}{0.87}            & 0.84  & \multicolumn{1}{l|}{0.89}              & 0.80    & \multicolumn{1}{l|}{0.85}          & 0.87          & \multicolumn{1}{l|}{0.86}              & 0.87    & \multicolumn{1}{l|}{0.85}          & 0.86          & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.89} \\ \hline
CWE-666                 & \multicolumn{1}{l|}{0.85}            & 0.84  & \multicolumn{1}{l|}{0.88}              & 0.86    & \multicolumn{1}{l|}{0.89}          & 0.90          & \multicolumn{1}{l|}{0.87}              & 0.92    & \multicolumn{1}{l|}{0.86}          & 0.91          & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.93} \\ \hline
CWE-665                 & \multicolumn{1}{l|}{0.83}            & 0.87  & \multicolumn{1}{l|}{0.90}              & 0.79    & \multicolumn{1}{l|}{0.93}          & 0.88          & \multicolumn{1}{l|}{0.92}              & 0.89    & \multicolumn{1}{l|}{0.92}          & 0.92          & \multicolumn{1}{l|}{\textbf{0.94}} & \textbf{0.92} \\ \hline
CWE-758                 & \multicolumn{1}{l|}{0.84}            & 0.87  & \multicolumn{1}{l|}{0.86}              & 0.83    & \multicolumn{1}{l|}{0.84}          & 0.88          & \multicolumn{1}{l|}{0.87}              & 0.92    & \multicolumn{1}{l|}{0.85}          & 0.89          & \multicolumn{1}{l|}{\textbf{0.91}} & \textbf{0.93} \\ \hline
CWE-469                 & \multicolumn{1}{l|}{0.75}            & 0.79  & \multicolumn{1}{l|}{0.78}              & 0.76    & \multicolumn{1}{l|}{\textbf{0.86}} & 0.83          & \multicolumn{1}{l|}{0.76}              & 0.79    & \multicolumn{1}{l|}{\textbf{0.83}} & 0.84          & \multicolumn{1}{l|}{0.83}          & \textbf{0.86} \\ \hline
CWE-676                 & \multicolumn{1}{l|}{0.84}            & 0.80  & \multicolumn{1}{l|}{0.84}              & 0.75    & \multicolumn{1}{l|}{\textbf{0.92}} & \textbf{0.91} & \multicolumn{1}{l|}{0.89}              & 0.83    & \multicolumn{1}{l|}{0.86}          & 0.89          & \multicolumn{1}{l|}{0.90}          & \textbf{0.91} \\ \hline
CWE-834                 & \multicolumn{1}{l|}{0.70}            & 0.62  & \multicolumn{1}{l|}{0.76}              & 0.74    & \multicolumn{1}{l|}{0.84}          & 0.79          & \multicolumn{1}{l|}{0.74}              & 0.72    & \multicolumn{1}{l|}{0.83}          & 0.76          & \multicolumn{1}{l|}{\textbf{0.87}} & \textbf{0.82} \\ \hline
CWE-79                  & \multicolumn{1}{l|}{0.82}            & 0.84  & \multicolumn{1}{l|}{0.84}              & 0.85    & \multicolumn{1}{l|}{0.85}          & 0.83          & \multicolumn{1}{l|}{0.86}              & 0.88    & \multicolumn{1}{l|}{0.86}          & 0.87          & \multicolumn{1}{l|}{\textbf{0.88}} & \textbf{0.90} \\ \hline
CWE-89                  & \multicolumn{1}{l|}{0.85}            & 0.82  & \multicolumn{1}{l|}{0.76}              & 0.80    & \multicolumn{1}{l|}{0.83}          & 0.85          & \multicolumn{1}{l|}{0.81}              & 0.84    & \multicolumn{1}{l|}{\textbf{0.87}} & 0.85          & \multicolumn{1}{l|}{\textbf{0.87}} & \textbf{0.87} \\ \hline
CWE-416                 & \multicolumn{1}{l|}{0.83}            & 0.85  & \multicolumn{1}{l|}{0.80}              & 0.81    & \multicolumn{1}{l|}{0.84}          & 0.87          & \multicolumn{1}{l|}{0.79}              & 0.84    & \multicolumn{1}{l|}{0.85}          & 0.88          & \multicolumn{1}{l|}{\textbf{0.88}} & \textbf{0.90} \\ \hline
CWE-20                  & \multicolumn{1}{l|}{0.84}            & 0.88  & \multicolumn{1}{l|}{0.80}              & 0.83    & \multicolumn{1}{l|}{0.87}          & 0.89          & \multicolumn{1}{l|}{0.86}              & 0.87    & \multicolumn{1}{l|}{0.89}          & 0.90          & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.92} \\ \hline
CWE-125                 & \multicolumn{1}{l|}{0.81}            & 0.85  & \multicolumn{1}{l|}{0.78}              & 0.83    & \multicolumn{1}{l|}{0.82}          & 0.87          & \multicolumn{1}{l|}{0.84}              & 0.84    & \multicolumn{1}{l|}{0.85}          & 0.86          & \multicolumn{1}{l|}{\textbf{0.86}} & \textbf{0.89} \\ \hline
\end{tabular}

}
\end{table*}


% \begin{table*}[t!]
% \caption{Results of the comparison with different baselines on SARD} 
% \label{tab:results}
% \scalebox{0.9}{
% \begin{tabular}{|l|ll|ll|ll|ll|ll|ll|}
% \hline
% \multirow{3}{*}{\diagbox[]{DataSet}{Metric}{Model}} & \multicolumn{2}{l|}{\multirow{2}{*}{DEVIGN}} & \multicolumn{2}{l|}{\multirow{2}{*}{LIN et al.}} & \multicolumn{2}{l|}{\multirow{2}{*}{FUNDED}}       & \multicolumn{2}{l|}{\multirow{2}{*}{DeepWukong}} & \multicolumn{2}{l|}{\multirow{2}{*}{$\tool_{noAnno}$}} & \multicolumn{2}{l|}{\multirow{2}{*}{\tool}}        \\
%                                & \multicolumn{2}{l|}{}                        & \multicolumn{2}{l|}{}                            & \multicolumn{2}{l|}{}                              & \multicolumn{2}{l|}{}                            & \multicolumn{2}{l|}{}                               & \multicolumn{2}{l|}{}                              \\ \cline{2-13} 
%                                & \multicolumn{1}{l|}{ACC}             & F1    & \multicolumn{1}{l|}{ACC}               & F1      & \multicolumn{1}{l|}{ACC}           & F1            & \multicolumn{1}{l|}{ACC}               & F1      & \multicolumn{1}{l|}{ACC}       & F1                 & \multicolumn{1}{l|}{ACC}           & F1            \\ \hline
% CWE-119                        & \multicolumn{1}{l|}{0.79}            & 0.81  & \multicolumn{1}{l|}{\textbf{0.85}}     & 0.78    & \multicolumn{1}{l|}{0.83}          & 0.85          & \multicolumn{1}{l|}{0.82}              & 0.84    & \multicolumn{1}{l|}{0.80}      & 0.86               & \multicolumn{1}{l|}{0.84}          & \textbf{0.87} \\ \hline
% CWE-400                        & \multicolumn{1}{l|}{\textbf{0.84}}   & 0.81  & \multicolumn{1}{l|}{0.79}              & 0.76    & \multicolumn{1}{l|}{\textbf{0.84}} & 0.80          & \multicolumn{1}{l|}{\textbf{0.84}}     & 0.79    & \multicolumn{1}{l|}{0.82}      & 0.83               & \multicolumn{1}{l|}{0.83}          & \textbf{0.85} \\ \hline
% CWE-404                        & \multicolumn{1}{l|}{0.84}            & 0.82  & \multicolumn{1}{l|}{0.83}              & 0.74    & \multicolumn{1}{l|}{0.81}          & 0.85          & \multicolumn{1}{l|}{0.83}              & 0.84    & \multicolumn{1}{l|}{0.83}      & 0.88               & \multicolumn{1}{l|}{\textbf{0.88}}          & \textbf{0.90} \\ \hline
% CWE-369                        & \multicolumn{1}{l|}{0.83}            & 0.78  & \multicolumn{1}{l|}{0.82}              & 0.80    & \multicolumn{1}{l|}{0.86}          & 0.84          & \multicolumn{1}{l|}{\textbf{0.91}}     & 0.87    & \multicolumn{1}{l|}{0.90}      & \textbf{0.91}      & \multicolumn{1}{l|}{0.89}          & 0.88          \\ \hline
% CWE-191                        & \multicolumn{1}{l|}{0.82}            & 0.76  & \multicolumn{1}{l|}{0.80}              & 0.73    & \multicolumn{1}{l|}{\textbf{0.87}} & 0.90          & \multicolumn{1}{l|}{0.75}              & 0.81    & \multicolumn{1}{l|}{0.81}      & 0.87               & \multicolumn{1}{l|}{0.85}          & \textbf{0.91} \\ \hline
% CWE-476                        & \multicolumn{1}{l|}{0.91}            & 0.87  & \multicolumn{1}{l|}{0.89}              & 0.83    & \multicolumn{1}{l|}{0.83}          & 0.87          & \multicolumn{1}{l|}{\textbf{0.90}}     & 0.86    & \multicolumn{1}{l|}{0.85}      & 0.84               & \multicolumn{1}{l|}{0.86}          & \textbf{0.89} \\ \hline
% CWE-467                        & \multicolumn{1}{l|}{0.79}            & 0.84  & \multicolumn{1}{l|}{0.87}              & 0.81    & \multicolumn{1}{l|}{0.85}          & 0.86          & \multicolumn{1}{l|}{0.88}              & 0.86    & \multicolumn{1}{l|}{0.86}      & 0.83               & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.87} \\ \hline
% CWE-78                         & \multicolumn{1}{l|}{0.82}            & 0.84  & \multicolumn{1}{l|}{\textbf{0.89}}     & 0.79    & \multicolumn{1}{l|}{0.83}          & \textbf{0.86} & \multicolumn{1}{l|}{0.84}              & 0.83    & \multicolumn{1}{l|}{0.84}      & 0.86               & \multicolumn{1}{l|}{0.85}          & 0.84          \\ \hline
% CWE-772                        & \multicolumn{1}{l|}{0.83}            & 0.77  & \multicolumn{1}{l|}{0.85}              & 0.81    & \multicolumn{1}{l|}{0.86}          & 0.87          & \multicolumn{1}{l|}{0.86}              & 0.83    & \multicolumn{1}{l|}{0.86}      & 0.88               & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.88} \\ \hline
% CWE-190                        & \multicolumn{1}{l|}{0.86}            & 0.83  & \multicolumn{1}{l|}{0.83}              & 0.79    & \multicolumn{1}{l|}{0.86}          & 0.84          & \multicolumn{1}{l|}{0.87}              & 0.83    & \multicolumn{1}{l|}{0.85}      & 0.82               & \multicolumn{1}{l|}{\textbf{0.92}} & \textbf{0.87} \\ \hline
% CWE-770                        & \multicolumn{1}{l|}{0.87}            & 0.84  & \multicolumn{1}{l|}{0.89}              & 0.80    & \multicolumn{1}{l|}{0.85}          & 0.87          & \multicolumn{1}{l|}{0.86}              & 0.87    & \multicolumn{1}{l|}{0.85}      & 0.86               & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.89} \\ \hline
% CWE-666                        & \multicolumn{1}{l|}{0.85}            & 0.84  & \multicolumn{1}{l|}{0.88}              & 0.86    & \multicolumn{1}{l|}{0.89}          & 0.90          & \multicolumn{1}{l|}{0.87}              & 0.92    & \multicolumn{1}{l|}{0.86}      & 0.91               & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.93} \\ \hline
% CWE-665                        & \multicolumn{1}{l|}{0.83}            & 0.87  & \multicolumn{1}{l|}{0.90}              & 0.79    & \multicolumn{1}{l|}{0.93}          & 0.88          & \multicolumn{1}{l|}{0.92}              & 0.89    & \multicolumn{1}{l|}{0.92}      & \textbf{0.92}      & \multicolumn{1}{l|}{\textbf{0.94}} & \textbf{0.92} \\ \hline
% CWE-758                        & \multicolumn{1}{l|}{0.84}            & 0.87  & \multicolumn{1}{l|}{0.86}              & 0.83    & \multicolumn{1}{l|}{0.84}          & 0.88          & \multicolumn{1}{l|}{0.87}              & 0.92    & \multicolumn{1}{l|}{0.85}      & 0.89               & \multicolumn{1}{l|}{\textbf{0.91}} & \textbf{0.93} \\ \hline
% CWE-469                        & \multicolumn{1}{l|}{0.75}            & 0.79  & \multicolumn{1}{l|}{0.78}              & 0.76    & \multicolumn{1}{l|}{\textbf{0.86}} & 0.83          & \multicolumn{1}{l|}{0.76}              & 0.79    & \multicolumn{1}{l|}{0.83}      & 0.84               & \multicolumn{1}{l|}{0.83}          & \textbf{0.86} \\ \hline
% CWE-676                        & \multicolumn{1}{l|}{0.84}            & 0.80  & \multicolumn{1}{l|}{0.84}              & 0.75    & \multicolumn{1}{l|}{\textbf{0.92}} & \textbf{0.91} & \multicolumn{1}{l|}{0.89}              & 0.83    & \multicolumn{1}{l|}{0.86}      & 0.89               & \multicolumn{1}{l|}{0.90}          & \textbf{0.91} \\ \hline
% CWE-834                        & \multicolumn{1}{l|}{0.70}            & 0.62  & \multicolumn{1}{l|}{0.76}              & 0.74    & \multicolumn{1}{l|}{0.84} & 0.79 & \multicolumn{1}{l|}{0.74}              & 0.72    & \multicolumn{1}{l|}{0.83}      & 0.76               & \multicolumn{1}{l|}{\textbf{0.87}}          & \textbf{0.82}          \\ \hline
% \end{tabular}
% }
% \end{table*}
\subsection{Performance Analysis on \textbf{SARD} (RQ1)}
We first verified the effectiveness of the proposed model and other baselines on a number of CWE vulnerability types, 
from which the models are trained and tested on \textbf{SARD} synthetic code samples. 
Note that the training and testing data ratio is 80\% and 70\%, respectively. 
Table~\ref{tab:results_25} reports the evaluation metrics on each vulnerability type. 
In general, even without incorporating the semantic meaning of \textcolor{red}{code comments} into the model (\tool$_{noAnno}$), 
our proposed model achieves promising results on almost all vulnerability types. 
\tool$_{noAnno}$ is the variant of \tool~only training on code representation graph using vulnerability oracle. 
Devign, Lin et al., DeepWukong, and \tool$_{noAnno}$ give low F1 and accuracy score on the CWE-834 dataset, 
which describes an ``\textit{Excessive Iteration}'' vulnerability that 
leads to the over-consumption of resources and can be adversely affected by attackers. 
This type of vulnerability presents no clear sign of vulnerable code patterns 
and is hardly identified by learning solely on code graph representations or code tokens. 
\tool, on the other hand, also leverages the semantic \textcolor{red}{code comment} information of the programs to enhance the robustness of the detection ability, 
thus achieving much better results compared with \tool$_{noAnno}$ and other baselines. 
It can also be observed that both Devign and Lin et al. perform undesirable on CWE-469, 
in which the vulnerability is caused by the misuse of the pointer variable. 
\tool~is the best-performing model on this dataset, 
indicating that the intra-program dependence in the CPG provides sufficient information when modelling the code graph in this case. 
FUNDED achieves marginal performance gain compared with \tool~and DeepWukong on CWE-676. 
We discover that this dataset relates to ``Use of Potentially Dangerous Function'' vulnerability, 
which can be identified by models capable of encoding control flow information. 
Therefore, FUNDED, DeepWukong and \tool~achieve similar results on this dataset. 
Lin et al. achieves the best Accuracy score on CWE-78, indicating high True Positive and Negative numbers. 
Yet it reports a low F1 score with poor results on Precision and Recall.
Overall, \tool~achieves the best results on most of the tested datasets, 
with an average 88.05\% on accuracy and 88.35\% on F1.


\textcolor{red}{
In order to more clearly and accurately demonstrate the advantages of the \tool, we also performed a quantitative analysis of the experiment data (Table \ref{tab:results_25}), using independent samples t-test.
We tested \tool~against DEVIGN, LIN et al., FUNDED, DeepWukong, and \tool$_{noAnno}$ separately.
In each test the comparisons were made separately for Accuracy and F1. The quantitative analysis is used to show whether \tool~is due to the comparison schemes.
We use $\tool.ACC$ to denote a set of experiment results.
Use $\Bar{X}_{\tool.ACC}$ to denote the mean of $\tool.ACC$, $S_{\tool.ACC}$ to denote the standard deviation, and $N_{\tool.ACC}$ to denote the number of samples:
}
\begin{equation}
\label{MeanDeviationNum}
\begin{split}
    & \textcolor{red}{\Bar{X}_{\tool.ACC}=\frac{1}{N_{\tool.ACC}}\sum^{N_{\tool.ACC}}_{i=1}\Bar{X}^{i}_{\tool.ACC}} \\
    & \textcolor{red}{S_{\tool.ACC}=\sqrt{\frac{1}{N_{\tool.ACC}-1}\sum^{N_{\tool.ACC}}_{i=1}(\Bar{X}^{i}_{\tool.ACC}-\Bar{X}_{\tool.ACC})^{2}}}
\end{split}
\end{equation}
\textcolor{red}{When we compare $DEVIGN.ACC$ and $\tool.ACC$, we can construct from the definition of the t-distribution:}
\begin{equation}
\label{MeanDeviationNum}
    \textcolor{red}{\frac{\Bar{X}_{\tool.ACC}-\Bar{X}_{DEVIGN.ACC}}{\sqrt{\frac{S^{2}_{\tool.ACC}}{N_{\tool.ACC}}+\frac{S^{2}_{DEVIGN.ACC}}{N_{DEVIGN.ACC}}}}\sim t(V)} 
\end{equation}
\textcolor{red}{
The degrees of freedom $V$ of this t-distribution are related to the degrees of freedom $V_{\tool.ACC}$  and $V_{DEVIGN.ACC}$:
}
\begin{equation}
\label{MeanDeviationNum}
    \textcolor{red}{V\approx\frac{(\frac{S^{2}_{\tool.ACC}}{N_{\tool.ACC}}+\frac{S^{2}_{DEVIGN.ACC}}{N_{DEVIGN.ACC}})^{2}}{\frac{S^{4}_{\tool.ACC}}{N^{2}_{\tool.ACC}\cdot V_{\tool.ACC}}+\frac{S^{4}_{DEVIGN.ACC}}{N^{2}_{DEVIGN.ACC}\cdot V_{DEVIGN.ACC}}}} 
\end{equation}
\textcolor{red}{We performed a quantitative analysis of the experimental results based on the aforementioned $\Bar{X}$, $S$, $V$ for the T-test, and the results are presented in Table \ref{tab:T-test}.}
\textcolor{red}{We first set a common significance level of 0.05 and degrees of freedom as 42.}
\textcolor{red}{Then we formulated two hypotheses and set a common significance level of 0.05:}
\begin{itemize}
    \item \textcolor{red}{Null Hypothesis (H0): There is no significant difference between the means of the two samples, i.e., $\mu1=\mu2$.}
    \item \textcolor{red}{Alternative Hypothesis (H1): There is a significant difference between the means of the two samples, i.e., $\mu1\neq \mu2$.}
\end{itemize}
\textcolor{red}{It can be observed that we can reject the Null Hypothesis and accept the Alternative Hypothesis except for F1 in comparsion of \tool and FUNDED, F1 in comparsion of \tool and DeepWukong and F1 in comparsion of \tool and DSHGTnoAnno.}
\textcolor{red}{In all three of above comparisons, we cannot quantitatively determine that \tool is better at a significance level of 0.05. However, our direct analysis of the results shows that \tool is superior to the comparison programs in these three metrics.}


\textcolor{red}{While the enhancement of the proposed method is modest in comparison to the baselines, our primary objective is to enhance the generalizability of our detection model, as evidenced by the subsequent experiments.	}

% \diagbox[]{Comparison}{T-test data}

\begin{table*}[t!]
\caption{\textcolor{red}{Results of T-test}} 
\label{tab:T-test}
\scalebox{0.7}{

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\diagbox[]{Comparison}{T-test data}                                &                      & Mean   & Standard deviation & T-value                 & Null Hypothesis(H0)  & Alternative Hypothesis(H1) \\ \hline
\multirow{4}{*}{\tool-DEVIGN}      & \multirow{2}{*}{ACC} & 0.8786 & 0.0329             & \multirow{2}{*}{2.0262} & \multirow{2}{*}{\XSolidBrush} & \multirow{2}{*}{\Checkmark}       \\ \cline{3-4}
                                   &                      & 0.8205 & 0.0489             &                         &                      &                            \\ \cline{2-7} 
                                   & \multirow{2}{*}{F1}  & 0.8791 & 0.0333             & \multirow{2}{*}{2.8975} & \multirow{2}{*}{\XSolidBrush} & \multirow{2}{*}{\Checkmark}       \\ \cline{3-4}
                                   &                      & 0.7909 & 0.0385             &                         &                      &                            \\ \hline
\multirow{4}{*}{\tool-LIN et al.}  & \multirow{2}{*}{ACC} & 0.8795 & 0.0337             & \multirow{2}{*}{2.2596} & \multirow{2}{*}{\XSolidBrush} & \multirow{2}{*}{\Checkmark}       \\ \cline{3-4}
                                   &                      & 0.8518 & 0.0274             &                         &                      &                            \\ \cline{2-7} 
                                   & \multirow{2}{*}{F1}  & 0.8845 & 0.0302             & \multirow{2}{*}{2.4167} & \multirow{2}{*}{\XSolidBrush} & \multirow{2}{*}{\Checkmark}       \\ \cline{3-4}
                                   &                      & 0.8586 & 0.0322             &                         &                      &                            \\ \hline
\multirow{4}{*}{\tool-FUNDED}      & \multirow{2}{*}{ACC} & 0.8827 & 0.0361             & \multirow{2}{*}{2.561}  & \multirow{2}{*}{\XSolidBrush} & \multirow{2}{*}{\Checkmark}       \\ \cline{3-4}
                                   &                      & 0.8331 & 0.0546             &                         &                      &                            \\ \cline{2-7} 
                                   & \multirow{2}{*}{F1}  & 0.8841 & 0.0367             & \multirow{2}{*}{1.520}  & \multirow{2}{*}{\Checkmark} & \multirow{2}{*}{\XSolidBrush}       \\ \cline{3-4}
                                   &                      & 0.8573 & 0.0388             &                         &                      &                            \\ \hline
\multirow{4}{*}{\tool-DeepWukong}  & \multirow{2}{*}{ACC} & 0.8645 & 0.0184             & \multirow{2}{*}{2.6197} & \multirow{2}{*}{\XSolidBrush} & \multirow{2}{*}{\Checkmark}       \\ \cline{3-4}
                                   &                      & 0.8486 & 0.0281             &                         &                      &                            \\ \cline{2-7} 
                                   & \multirow{2}{*}{F1}  & 0.8841 & 0.0367             & \multirow{2}{*}{1.520}  & \multirow{2}{*}{\Checkmark} & \multirow{2}{*}{\XSolidBrush}       \\ \cline{3-4}
                                   &                      & 0.8361 & 0.0517             &                         &                      &                            \\ \hline
\multirow{4}{*}{\tool-DSHGTnoAnno} & \multirow{2}{*}{ACC} & 0.8682 & 0.018              & \multirow{2}{*}{2.6006} & \multirow{2}{*}{\XSolidBrush} & \multirow{2}{*}{\Checkmark}       \\ \cline{3-4}
                                   &                      & 0.8536 & 0.0197             &                         &                      &                            \\ \cline{2-7} 
                                   & \multirow{2}{*}{F1}  & 0.8800 & 0.012              & \multirow{2}{*}{1.3149} & \multirow{2}{*}{\Checkmark} & \multirow{2}{*}{\XSolidBrush}       \\ \cline{3-4}
                                   &                      & 0.8636 & 0.0194             &                         &                      &                            \\ \hline
\end{tabular}




}
\end{table*}





\begin{figure}[t!]
\centering
\includegraphics[width=0.5\linewidth]{figs/codesample.png}
\captionsetup{justification=centering}
\caption{Both C/C++ and Java code samples with ``OS Command Injection'' vulnerability on CWE-78.}
\label{fig:codesample}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.97\linewidth]{figs/transfer_without_python_new.png}
\captionsetup{justification=centering}
\caption{\textcolor{red}{Knowledge transferring capability \\from C/C++ to other programming languages}}
\label{fig:transfer}
\end{figure}



\subsection{Transferability on Other Programming Languages (RQ2)}
We experimented with the transferring capability of our proposed model against other baselines. 
To achieve that, we adopted the transfer learning technique by keeping the model structure and weights trained on C/C++ dataset, 
and fine-tuned that on other programming languages for vulnerability detection tasks. 
It is proven feasible in~\cite{funded} that the model trained in one programming languages domain 
can preserve the knowledge of vulnerable code patterns and thus be used to detect the similar vulnerabilities in other programming languages.

In this case, we first trained our model and other baselines on CWE-78 of C/C++ datasets. 
To transfer the knowledge learned from C/C++, 
we only fine-tuned the final MLP classifier of each model (2 linear layers and 1 output layer) for 10 epochs. 
We consider two cases that use transfer learning, C/C++ to Java and C/C++ to PHP. 
% \textcolor{red}{Only CWE-78 contains code fragments of both C/C++, Java and PHP}
Figure~\ref{fig:transfer} shows the result of the models' transferability \textcolor{red}{on CWE-78, CWE-79 and CWE-89}. 
It can be observed that our pre-trained model can better capture the prior vulnerable code patterns 
and achieve promising results when applied to other programming languages, 
with 84\% accuracy from C to Java and 88\% accuracy from C to PHP. 
%
We further explored the rationale behind the effectiveness of using transfer learning. 
It can be observed from Figure~\ref{fig:codesample} that both C/C++ and Java code samples 
in CWE-78 construct an OS command (highlighted in red) using externally-influenced input 
from an upstream component without validating the special element that could harm the system, 
thus are under threat of command inject attacks. 
%
In the CPG of both code samples, a control flow edge should exist if this command variable is validated before being used by other threads, 
thus presenting a similar code pattern regardless of language syntax. 
The result verifies that our model can better capture both contextual semantics 
and underlying structure (syntax, control- and data-flow) of the codes with the help of CPG and the corresponding heterogeneous graph learning, 
thus able to preserve the language-agnostic vulnerable code patterns. 




\begin{figure}[t!]
\centering
\includegraphics[width=0.5\linewidth]{figs/ast.png}
\captionsetup{justification=centering}
\caption{\textcolor{red}{Results on different code graph representations}}
\label{fig:representations}
\end{figure}



% \begin{table}[t!]
% \caption{Results on different code graph representations} 
% \label{tab:results_cpg}
% \scalebox{0.8}{
% \begin{tabular}{|ll|l|}
% \hline
% \multicolumn{2}{|l|}{\diagbox[innerwidth=3.6cm]{Code Representation}{Metric}{DataSet}}                  & CWE-119 \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{AST}}     & ACCURACY  & 0.68    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & PRECISION & 0.72    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & RECALL    & 0.57    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & F1        & 0.64    \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{PDG}}     & ACCURACY  & 0.79    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & PRECISION & 0.81    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & RECALL    & 0.70    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & F1        & 0.75    \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{AST+CFG}} & ACCURACY  & 0.81    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & PRECISION & 0.83    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & RECALL    & 0.73    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & F1        & 0.78    \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{AST+PDG}} & ACCURACY  & 0.85    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & PRECISION & 0.89    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & RECALL    & 0.74    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & F1        & 0.83    \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{CPG}}     & ACCURACY  & 0.83    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & PRECISION & 0.92    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & RECALL    & 0.79    \\ \cline{2-3} 
% \multicolumn{1}{|l|}{}                         & F1        & 0.86    \\ \hline
% \end{tabular}
% }
% \end{table}








\begin{table}[t]
\captionsetup{justification=centering}
\caption{Analysis on HGT layer \\and training time cost on CWE-119}
\label{tab:hgtlayer}
\scalebox{0.85}{
\begin{tabular}{|l|lllll|}
\hline
\multirow{2}{*}{Metric} & \multicolumn{5}{c|}{HGT Layer Depths}                                                                                   \\ \cline{2-6} 
                        & \multicolumn{1}{l|}{1}    & \multicolumn{1}{l|}{2}    & \multicolumn{1}{l|}{3}     & \multicolumn{1}{l|}{4}     & 5     \\ \hline
F1                      & \multicolumn{1}{l|}{0.79} & \multicolumn{1}{l|}{0.87} & \multicolumn{1}{l|}{0.89}  & \multicolumn{1}{l|}{0.88}  & 0.85  \\ \hline
Training Time Cost/h    & \multicolumn{1}{l|}{4.83} & \multicolumn{1}{l|}{9.45} & \multicolumn{1}{l|}{14.88} & \multicolumn{1}{l|}{19.81} & 23.64 \\ \hline
\end{tabular}
}
\end{table}

\begin{table*}[t!]
\caption{Ablation study on graph learning and non-graph learning on CPG} 
\label{tab:hete}
\scalebox{0.9}{
\begin{tabular}{|ll|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\diagbox[innerwidth=4.9cm]{Model}{Metric}}                                      & ACCURACY & PRECISION & RECALL & F1   \\ \hline
\multicolumn{1}{|l|}{w/o graph-based learning}               & BiLSTM     & 0.72     & 0.74      & 0.65   & 0.69 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{graph-based learning}} & $HGT_{homo}$  & 0.79     & 0.80      & 0.68   & 0.74 \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                                     & $HGT_{heter}$ & 0.83     & 0.92      & 0.79   & 0.86 \\ \hline
\end{tabular}
}
\end{table*}

\begin{table*}[t!]
\caption{Results of the comparison with different baselines on real-world projects}
\label{tab:realworld}
\scalebox{0.9}{
\begin{tabular}{|ll|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{\diagbox[innerwidth=4cm]{DataSet}{Metric}{Model}}                & DEVIGN & LIN et al. & DeepWukong & FUNDED & DSHGT \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{FFmpeg}} & ACCURACY  & 0.74   & 0.64       & 0.75       & 0.75   & 0.79 \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                        & PRECISION & 0.81   & 0.72       & 0.79       & 0.83   & 0.86 \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                        & RECALL    & 0.68   & 0.58       & 0.71       & 0.67   & 0.73 \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                        & F1        & 0.70   & 0.66       & 0.78       & 0.79   & 0.84 \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{QEMU}}   & ACCURACY  & 0.73   & 0.60       & 0.72       & 0.72   & 0.78 \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                        & PRECISION & 0.78   & 0.70       & 0.80       & 0.76   & 0.84 \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                        & RECALL    & 0.69   & 0.54       & 0.69       & 0.68   & 0.73 \\ \cline{2-7} 
\multicolumn{1}{|l|}{}                        & F1        & 0.74   & 0.64       & 0.75       & 0.73   & 0.82 \\ \hline
\end{tabular}
}
\end{table*}


\begin{figure}[t!]
\centering
\includegraphics[width=1\linewidth]{figs/sensitivity-new.png}
\caption{\textcolor{red}{Change of Acc and F1 along with $\lambda$ on CWE-119, CWE-190 and CWE-476}}
\label{fig:sensitivity}
\end{figure}


\subsection{Impact of Dual-supervisors (RQ3)}
\label{sec:rq3}
To answer RQ3, we studied the necessity of designing multi-task learning with dual supervisors 
to enhance the performance of \tool~as well as how to balance between two supervisors responsible 
for dealing with the vulnerability label oracle and the \textcolor{red}{code comment} oracle, 
in which the textual \textcolor{red}{code comments} are used as supplementary information. 
Note the use of auxiliary annotations of code snippets is proven helpful for tasks like code completion~\cite{annotation1}, 
code summarization~\cite{annotation2}, and code retrival~\cite{annotation3}. 
We thus hypothesize that the graph code embedding should contain rich semantic information capable of summarizing the code snippets in \textcolor{red}{code comment} formats. 
In the experiment, the sensitivity of $\lambda$ is explored to control the level of impact caused by contextual \textcolor{red}{code comments} when training the model, 
in which 0 indicates only training the model based on vulnerability labels, 
while 1 means only optimizing the model towards generating correct \textcolor{red}{code comment} summaries of codes (reflected in Eq.13). 
We first experiment on the HGT layer depth and compare the change of layer depth against detection performance and mode training cost. 
It is shown in Table~\ref{tab:hgtlayer} that the time cost increases with the increase of HGT layer depths, and F1 reaches the highest when layer depth is 3. 
We thus choose 3 as the layer depth setup for HGT. Regarding the sensitivity of $\lambda$, \textcolor{red}{we conducted experiments on CWE-119, CWE-190, CWE-476.} Figure~\ref{fig:sensitivity} reveals the change of Accuracy and F1 scores along with $\lambda$. 
Both scores \textcolor{red}{on three datasets} reach the highest when $\lambda$ = 0.2 and decrease afterwards on, 
indicating that over-reliance on \textcolor{red}{code comments} aggravates the vulnerability detection ability 
subject to the quality and number of \textcolor{red}{code comments} in the programs, 
while using semantic information in \textcolor{red}{code comments} is beneficial to some extent. 
It is not uncommon to have a mixture of good and bad \textcolor{red}{code comments} in the program. 
Taking CWE-119 as an example, we discover that some \textcolor{red}{code comments} 
like ``\textit{fixes the problem of not freeing the data in the source}'' have specific meanings or descriptions for the method, 
the semantics of which are then comprehended into the graph-level embedding through 
the training process and become helpful for determining whether the method is vulnerable, 
while there exist \textcolor{red}{some code comments} like ``\textit{use goodsource 
and badsink by changing the first GLOBAL\_CONST\_TRUE to GLOBAL\_CONST\_FALSE}'', which are not helpful. 
Over-reliance on such \textcolor{red}{code comments} thus (large $\lambda$) deteriorates the vulnerability detection performance.   


\subsection{Ablation Study (RQ4)}

We first investigate the use of AST, PDG, AST+CFG, and AST+PDG as different code graph representations, 
aiming to check the effectiveness of using CPG. As shown \textcolor{red}{Figure}~\ref{fig:representations}, 
the model trained by AST-based graphs generates the worst results, 
meaning the sole syntax information is insufficient when detecting the code's vulnerabilities. 
In general, using heterogeneous code graph representations such as AST+CFG and AST+PDG produces better results than using AST and PDG separately, 
and CPG achieves the best results among all as it combines properties of AST, CFG and PDG.

Additionally, we explore the importance of heterogeneous graph learning when it comes to encoding the CPG. 
As pointed out in the previous section, the core component of enabling heterogeneous graph learning is HGT, 
which presents good performance when incorporating the 
large number neighbors of different types, 
\textit{i.e.}, complex node and edge heterogeneity in the graph structure~\cite{hu2020heterogeneous}. 
To answer this, we implemented HGT$_{homo}$, which is the variant of HGT and only maintains 
a single set of parameters for all relations (e.g., $Q{\text{-}}Linear$, $K{\text{-}}Linear$ and $V{\text{-}}Linear$ matrices share same parameters regardless of types). 
By doing so, HGT$_{homo}$ preserves the graph learning ability while ignoring the various node/edge types in the CPG. 
It can be seen clearly that HGT$_{heter}$ demonstrates a significant performance gain across all metrics, 
proving the great importance of encoding the structural heterogeneity of the program graphs. 
Specifically, HGT$_{heter}$ keeps distinct edge-based metrics $W^{ATT}_{\phi(e)}$ and $W^{MSG}_{\phi(e)}$ for each edge type $\phi(e)$, 
which enables the model to distinguish the semantic differences of relations even between the same node types. 
Additionally, the edge-driven attention mechanism allows the target node to measure the importance of each connected source node with different edge types. 
For instance, in the case of buffer overflow vulnerability in CWE-119, 
the falsely converted \textit{unsign} length variable (source node) 
by \textit{atoi} contributes more to the \textit{memcpy} method (target node) with a larger attention value over the data dependency edge type. 
The importance of this \textit{unsign} variable's node embedding will eventually reflect in the graph-level embedding through readout operation, 
which then helps downstream vulnerability detection task.
Apart from that, we also study the role of graph learning in the experiment. 
Similar to ~\cite{sysevr,lin}, we use BiLSTM as the alternative to encode the code snippets, 
which tokenizes the code representation (i.e., CPG in this case) as input while ignoring the syntax, semantics, and flows structure information in the graphs. 
The experimental results show that HGT$_{heter}$ outperforms BiLSTM with a greater 10\% performance gain, 
manifesting the significance of incorporating structure information when modelling the code snippets.


\subsection{Results on Real-world Open Source Projects (RQ5)}

We verify the effectiveness of our proposed framework and other baselines 
on real-world programs extracted from C/C++ open-source projects \textbf{\textit{FFmpeg}} and \textbf{\textit{QEMU}}. 
The detailed statistics of these projects 
are shown in Table~\ref{tab:dataset}.

Table~\ref{tab:realworld} records the experimental results on these projects. 
In general, we observe a drop in performance for both our proposed framework and other baselines on real-world open projects, 
as there are much fewer labeled vulnerable samples in these two projects than synthetic code samples in \textbf{SARD}. 
This attributes to the existence of vulnerability label noise in both FFmpeg and QEMU since the function-level vulnerabilities are labelled based
on determining vulnerability-fix commits or non-vulnerability fix commits of
these projects. Additionally, Lin et al. underperform for all metrics, especially for \textbf{Recall} (high volumes of false-negative predictions), 
suggesting that only using code tokens in the program to train the detection model is insufficient nor applicable to real-world projects. 
Other baselines present results with marginal differences, while \tool~outperforms all of them. 
We discover that both projects contain a large number of fixes for vulnerabilities such as \textit{Memory Leak} and \textit{Buffer Overflow}, 
 which require to better encode the information of different edge types (control flow and dependency information) into the graph-level embedding for better detection results. 
 \tool~learns on the CPG without losing the heterogeneity attributes, 
 thus is more generalized even on real-world projects. 
 Overall, \tool~delivers the best performance for 
\textbf{Accuracy} (7.9\% improvement on average), 
\textbf{Precision} (7.65\% improvement on average), 
\textbf{Recall} (7.5\% improvement on average) 
and 
\textbf{F1} (10.6\% improvement on average). A promising way to improve the performance on real-world projects is to adapt state-of-the-art zero-shot or few-shot learning specifically for heterogeneous graph networks.


\section{Threat to Validity}
\label{sec:validity}

\textbf{External validity}:
In our experiments, we chose 4 baselines: 
\textbf{LIN \textit{et al.}}~\cite{lin},
\textbf{DEVIGN}~\cite{devign}, 
\textbf{FUNDED}~\cite{funded} 
and 
\textbf{DeepWukong}~\cite{deepwukong}. 
We believe these 4 baselines could represent the state-of-the-art research outputs, 
including non-graph learning methods for code tokens and graph learning methods for code graph representations.
%
%
For the datasets used, we used 17 categories of C/C++, Java and PHP from \textbf{SARD}, 
which shall cover the most commonly seen vulnerability types.
%
Due to the lack of labeled vulnerabilities datasets from real-world projects, 
we could only evaluate \tool~on the real-world open-source projects 
(\textit{i.e.} \textbf{\textit{FFmpeg}} and \textbf{\textit{QEMU}}, 
which has also been used by~\cite{li2021vuldeelocator},~\cite{lin} and~\cite{devign}).
As these two projects also allow code contributions, 
we believe they are good representations of state-of-the-art real-world projects. 
Even though our proposed \tool~has shown the transferability to detect Java and PHP vulnerabilities after being trained on the C/C++ dataset, 
the vulnerability datasets for programming languages other than C/C++ are still limited. 
We will continue to work on this issue and build up related datasets for future usage in this community.

\noindent\textbf{Internal validity}:
The quality of \textcolor{red}{code comments} used for training might not align with the ground truth perfectly due to the semantic complexity of codes and human errors.
As discussed in Section~\ref{sec:rq3}, the hand-written \textcolor{red}{code comment} highly relies on the programmers' personal habits,
and different programmers could provide different \textcolor{red}{code comments} for the same source code segment.
Thus, we do not rely heavily on the \textcolor{red}{code comment} supervisor, 
and our empirical study shows that our \tool~reaches the highest performance when $\lambda = 0.2$. 
We plan to use \tool~in the future for those real-world software projects where 
we have finer-granularity control of the \textcolor{red}{code comment} quality to remove the confounding variables such as human errors or other noises.

\noindent\textbf{Construct validity}
The layer depth of \textit{HGT} in \textit{DSHGT} is set to 3 based on the empirical study result (as shown in Section~\ref{sec:rq3}). 
The target node embedding is updated through the attentive message passing from neighbor nodes.
As the layer numbers increase, the \textit{HGT} will eventually face the oversmoothing problem~\cite{chen2020measuring}, 
where distinct information conveyed by neighbors become hard to distinguish owing to the over-iterative message passing, and leads to performance degradation.
%
We leverage a simple 1 layer LSTM as the decoder for the \textcolor{red}{code comment} supervisor part, 
which already demonstrates promising results in the experiment. 
It suggests the potential of using auxiliary \textcolor{red}{code comments} as supplementary information to assist the vulnerability detection task. 
As a future task, we can leverage more calibrated semantic extraction models 
such as those pretrained NLP models~\cite{kalyan2021ammus} as the \textcolor{red}{code comment} decoder. 




\section{Conclusion}
\label{sec:conclusion}

In this paper, we present our pioneer study of using heterogeneous graph learning for detecting software vulnerabilities. 
In this work, we have chosen to use CPG as the heterogeneous graph and customized a dual-supervisor graph learning model. 
The extensive experiments on synthetic and real-world software projects show promising results. 
We are one of the first to explore the importance of conducting research in heterogeneous graph learning 
to detect software vulnerability for the software engineering community. 
Besides good results in different programming languages and real-world projects, 
software engineers can leverage the largely open-sourced new results from graph learning 
and NLP communities to further enhance this line of research to have better heterogeneous graph representation other than CPG, 
leverage more robust learning models for latent features in the underlying heterogeneous graph, 
and utilize more reliable and controllable supervisors in addition to the binary vulnerability oracle.


% %%
% %% The acknowledgments section is defined using the "acks" environment
% %% (and NOT an unnumbered section). This ensures the proper
% %% identification of the section in the article metadata, and the
% %% consistent spelling of the heading.
% \begin{acks}
% To Robert, for the bagels and explaining CMYK and color spaces.
% \end{acks}

\clearpage
\bibliographystyle{ACM-Reference-Format}
\bibliography{ref}

%%
%% If your work has an appendix, this is the place to put it.

% \printbibliography
% \bibliographystyle{ACM-Reference-Format}
% \bibliography{ref}


%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.


% \begin{acks}
% To Robert, for the bagels and explaining CMYK and color spaces.
% \end{acks}


% %%
% %% Print the bibliography
% %%
% \printbibliography

% %%
% %% If your work has an appendix, this is the place to put it.
% \appendix






\clearpage
\onecolumn


\section{Appendix}

\label{sec:app}
We show supplementary tables in this Appendix.


\begin{table}[h!]
\centering
\caption{All node types in CPG.}
\label{tab:node}
\scalebox{0.55}{
\begin{tabular}{|l|l|}
\hline
node\_type                    & description                                                                                                                     \\ \hline
META\_DATA                    & This node contains the CPG meta data.                                                                                           \\ \hline
FILE                          & File nodes represent source files or a shared objects from which the CPG was generated.                                         \\ \hline
NAMESPACE                     & This node represents a namespace.                                                                                               \\ \hline
NAMESPACE\_BLOCK              & A reference to a namespace.                                                                                                     \\ \hline
METHOD                        & This node represents procedures, functions, methods.                                                                            \\ \hline
METHOD\_PARAMETER\_IN         & This node represents a formal input parameter.                                                                                  \\ \hline
METHOD\_PARAMETER\_OUT        & This node represents a formal output parameter.                                                                                 \\ \hline
METHOD\_RETURN                & This node represents an (unnamed) formal method return parameter.                                                               \\ \hline
MEMBER                        & This node represents a type member of a class, struct or union.                                                                 \\ \hline
TYPE                          & This node represents a type instance, a concrete instantiation of a type declaration.                                           \\ \hline
TYPE\_ARGUMENT                & This node represents a type argument which is used to instantiate a parametrized type.                                          \\ \hline
TYPE\_DECL                    & This node represents a type declaration.                                                                                        \\ \hline
TYPE\_PARAMETER               & This node represents a formal type parameter,  the type parameter as given in a type-parametrized method or type declaration.   \\ \hline
AST\_NODE                     & This is the base type for all nodes of the abstract syntax tree (AST).                                                          \\ \hline
BLOCK                         & This node represents a compound statement.                                                                                      \\ \hline
CALL                          & A (function/method/procedure) call.                                                                                             \\ \hline
CALL\_REPR                    & This is the base class of  CALL.                                                                                                \\ \hline
CONTROL\_STRUCTURE            & This node represents a control structure as introduced by control structure statements.                                         \\ \hline
EXPRESSION                    & This node is the base class for all nodes that represent code pieces that can be evaluated.                                     \\ \hline
FIELD\_IDENTIFIER             & This node represents the field accessed in a field access.                                                                      \\ \hline
IDENTIFIER                    & This node represents an identifier as used when referring to a variable by name..                                               \\ \hline
JUMP\_LABEL                   & This node specifies the label and thus the JUMP\_TARGET of control structures BREAK and CONTINUE.                               \\ \hline
JUMP\_TARGET                  & A jump target is a location that has been specifically marked as the target of a jump.                                          \\ \hline
LITERAL                       & This node represents a literal such as an integer or string constant.                                                           \\ \hline
LOCAL                         & This node represents a local variable.                                                                                          \\ \hline
METHOD\_REF                   & This node represents a reference to a method/function/procedure as it appears when a method is passed as an argument in a call. \\ \hline
MODIFIER                      & This node represents a (language-dependent) modifier such as `static', `private' or `public'.                                   \\ \hline
RETURN                        & This node represents a return instruction.                                                                                      \\ \hline
TYPE\_REF                     & Reference to a type/class.                                                                                                      \\ \hline
UNKNOWN                       & This node represents an AST node but there is no suitable AST node type.                                                        \\ \hline
CFG\_NODE                     & Base class for all control flow nodes.                                                                                          \\ \hline
COMMENT                       & A source code comment node.                                                                                                     \\ \hline
FINDING                       & Finding nodes are used to store analysis results in the graph.                                                                  \\ \hline
KEY\_VALUE\_PAIR              & This node represents a key-value pair.                                                                                          \\ \hline
LOCATION                      & A location node summarizes a source code location.                                                                              \\ \hline
TAG                           & This node represents a tag.                                                                                                     \\ \hline
TAG\_NODE\_PAIR               & This node contains an arbitrary node and an associated tag node.                                                                \\ \hline
CONFIG\_FILE                  & This node represent a configuration file.                                                                                       \\ \hline
BINDING                       & BINDING nodes represent name-signature pairs that can be resolved at a type declaration.                                        \\ \hline
ANNOTATION                    & A method annotation node.                                                                                                       \\ \hline
ANNOTATION\_LITERAL           & A literal value assigned to an ANNOTATION\_PARAMETER.                                                                           \\ \hline
ANNOTATION\_PARAMETER         & Formal annotation parameter.                                                                                                    \\ \hline
ANNOTATION\_PARAMETER\_ASSIGN & Assignment of annotation argument to annotation parameter.                                                                      \\ \hline
ARRAY\_INITIALIZER            & Initialization construct for arrays.                                                                                            \\ \hline
DECLARATION                   & Base node class for all declarations.                                                                                           \\ \hline
\end{tabular}
}
\end{table}



\begin{table}[h!]
\centering
\caption{All edge types in CPG.}
\label{tab:edge}
\scalebox{0.55}{
\begin{tabular}{|l|l|}
\hline
edge\_type      & description                                                                                                                                        \\ \hline
SOURCE\_FILE    & This edge connects a node to the node that represents its source file.                                                                             \\ \hline
ALIAS\_OF       & This edge represents an alias relation between a type declaration and a type.                                                                      \\ \hline
BINDS\_TO       & This edge connects type arguments to type parameters to indicate that the type argument is used to instantiate the type parameter.                 \\ \hline
INHERITS\_FROM  & Inheritance relation between a type declaration and a type.                                                                                        \\ \hline
AST             & This edge connects a parent node to its child in the abstract syntax tree.                                                                         \\ \hline
CONDITION       & The edge connects control structure nodes to the expressions that holds their conditions.                                                          \\ \hline
ARGUMENT        & Argument edges connect call sites to their arguments as well as the expressions that return.                                                       \\ \hline
CALL            & This edge connects call sites.                                                                                                                     \\ \hline
RECEIVER        & RECEIVER edges connect call sites to their receiver arguments.                                                                                     \\ \hline
CFG             & This edge indicates control flow from the source to the destination node.                                                                          \\ \hline
DOMINATE        & This edge indicates that the source node immediately dominates the destination node.                                                               \\ \hline
POST\_DOMINATE  & This edge indicates that the source node immediately post dominates the destination node.                                                          \\ \hline
CDG             & A CDG edge expresses that the destination node is control dependent on the source node.                                                            \\ \hline
REACHING\_DEF   & A reaching definition edge indicates that a variable produced at the source node reaches the destination node without being reassigned on the way. \\ \hline
CONTAINS        & This edge connects a node to the method that contains it.                                                                                          \\ \hline
EVAL\_TYPE      & This edge connects a node to its evaluation type.                                                                                                  \\ \hline
PARAMETER\_LINK & This edge connects a method input parameter to the corresponding method output parameter.                                                          \\ \hline
TAGGED\_BY      & This edge connects a node to the a TAG node.                                                                                                       \\ \hline
BINDS           & This edge connects a type declaration (TYPE\_DECL) with a binding node (BINDING).                                                                  \\ \hline
REF             & This edge indicates that the source node is an identifier that denotes access to the destination node.                                             \\ \hline
\end{tabular}
}
\end{table}



\begin{table}[t!]
\centering
\caption{Dataset Overview}
\label{tab:dataset}
\scalebox{0.47}{
\begin{tabular}{|l|l|l|l|l|}
\hline
Language                                          & Vul Category & Description                                                                                                                                                                                                                                & Vulnerable Samples & Non-vulnerable Samples \\ \hline
\multirow{17}{*}{C/C++}                           & CWE-119      & Improper Restriction of Operations within the Bounds of a Memory Buffer                                                                                                                                                                    & 1597               & 5406                   \\ \cline{2-5} 
                                                  & CWE-400      & Uncontrolled Resource Consumption                                                                                                                                                                                                          & 2786               & 8563                   \\ \cline{2-5} 
                                                  & CWE-404      & Improper Resource Shutdown or Release                                                                                                                                                                                                      & 1054               & 3748                   \\ \cline{2-5} 
                                                  & CWE-369      & Divide By Zero                                                                                                                                                                                                                             & 2691               & 8266                   \\ \cline{2-5} 
                                                  & CWE-191      & Integer Underflow (Wrap or Wraparound)                                                                                                                                                                                                     & 3473               & 10572                  \\ \cline{2-5} 
                                                  & CWE-476      & NULL Pointer Dereference                                                                                                                                                                                                                   & 1467               & 7336                   \\ \cline{2-5} 
                                                  & CWE-78       & \begin{tabular}[c]{@{}l@{}}Improper Neutralization of Special Elements used in an OS Command\\  (`OS Command Injection')\end{tabular}                                                                                                      & 10519              & 37854                  \\ \cline{2-5} 
                                                  & CWE-772      & Missing Release of Resource after Effective Lifetime                                                                                                                                                                                       & 4755               & 11847                  \\ \cline{2-5} 
                                                  & CWE-467      & Use of sizeof(~) on a Pointer Type                                                                                                                                                                                                          & 867                & 3573                   \\ \cline{2-5} 
                                                  & CWE-190      & Integer Overflow or Wraparound                                                                                                                                                                                                             & 3648               & 10487                  \\ \cline{2-5} 
                                                  & CWE-770      & Allocation of Resources Without Limits or Throttling                                                                                                                                                                                       & 843                & 2973                   \\ \cline{2-5} 
                                                  & CWE-666      & Operation on Resource in Wrong Phase of Lifetime                                                                                                                                                                                           & 1321               & 4589                   \\ \cline{2-5} 
                                                  & CWE-665      & Improper Initialization                                                                                                                                                                                                                    & 1436               & 4680                   \\ \cline{2-5} 
                                                  & CWE-758      & Reliance on Undefined, Unspecified, or Implementation-Defined Behavior                                                                                                                                                                     & 1674               & 5745                   \\ \cline{2-5} 
                                                  & CWE-469      & Use of Pointer Subtraction to Determine Size                                                                                                                                                                                               & 667                & 2745                   \\ \cline{2-5} 
                                                  & CWE-676      & Use of Potentially Dangerous Function                                                                                                                                                                                                      & 478                & 1394                   \\ \cline{2-5} 
                                                  & CWE-834      & Excessive Iteration                                                                                                                                                                                                                        & 362                & 1644                   \\ \hline
JAVA                                              & CWE-78       & \begin{tabular}[c]{@{}l@{}}Improper Neutralization of Special Elements used in an OS Command \\ (`OS Command Injection')\end{tabular}                                                                                                      & 476                   & 1576                       \\ \hline
PHP                                               & CWE-78       & \begin{tabular}[c]{@{}l@{}}Improper Neutralization of Special Elements used in an OS Command \\ (`OS Command Injection')\end{tabular}                                                                                                      & 268                   &  473                      \\ \hline
\multirow{2}{*}{Real-World  Open Source Projects} & FFmpeg       & \begin{tabular}[c]{@{}l@{}}FFmpeg is a software for handling video, audio, and other multimedia files and streams. \\ Its major vulnerability type is overflow vulnerability.\end{tabular}                                                 & 4981               & 4788                   \\ \cline{2-5} 
                                                  & QEMU         & \begin{tabular}[c]{@{}l@{}}QEMU is a hardware virtualization software, and its main vulnerability types include DoS attacks, \\ code execution vulnerabilities caused by overflows, and privilege escalation vulnerabilities.\end{tabular} & 7479               & 10070                  \\ \hline
\end{tabular}
}
\end{table}





























==> Casestudy.tex <==
.



==> Challenge.tex <==
%Testing learning-enabled CPS significantly differs from testing traditional software systems due to several key distinctions. Traditional software testing relies on well-defined specifications and coverage metrics, such as statement coverage, function coverage, and branch coverage, to guide the testing process and measure its effectiveness. However, defining coverage metrics for machine learning models within a learning-enabled CPS is a significant challenge. Determining the concept of ``full coverage'' testing for a neural network is intricate, and current coverage-driven approaches are considerably limited~\cite{harel2020neuron,li2019structural,yang2022revisiting,usman2022overview} (\textbf{Coverage Metrics Challenge}). Traditional software testing often employs an ``oracle'' – a benchmark for expected outcomes to compare against actual results. In learning-enabled CPS, however, such oracles might be absent, especially when it comes to assessing the quality of labels in training data for machine learning models. Unlike the manual test cases typical of conventional software testing, evaluating the label quality in learning-enabled CPS demands a thorough examination of the datasets used for training. These datasets, often vast in volume, can be multi-modal and high-dimensional. Ensuring the accuracy and consistency of labels within them presents unique and intricate challenges (\textbf{Oracle Challenge}). Furthermore, in traditional software, behavior is generally fixed once deployed unless manually updated or patched. In contrast, a learning-enabled CPS may continuously learn and adapt its behavior over time based on new data, making the testing and validation process ongoing and dynamically changing (\textbf{Behavior Change Challenge}). 
Recently, there has been a notable increase in research that concentrates on the formal verification of machine learning models. Various techniques have been employed, such as geometric reachability through NNV star sets~\cite{tran2020verification}, mixed-integer programming feasibility via Sherlock~\cite{dutta2019sherlock}, SMT solvers like Reluplex~\cite{katz2017reluplex}, and model-free optimization methods like Branch and Bound~\cite{bunel2018unified}. While this body of work primarily aims at ensuring the robustness and safety of individual models, it commonly falls short in several areas. One significant limitation is the tendency to treat robustness as a function of a predefined geometric input space. Within this space, researchers typically search for a 'radius' where the model's predictions remain stable or are bounded by linear constraints. Additionally, while recent neural network verification competitions~\cite{bak2021second} have started to explore practical issues, such as the prevention of aircraft collisions~\cite{owen2019acas}, these efforts often lack alignment with formally specified safety requirements, like those defined in Signal Temporal Logic~\cite{donze2010robust}. Moreover, the target systems under study frequently comprise single, relatively simplistic models. These lack the complexity, both in terms of input spaces and architecture, that one encounters in industry-scale, multi-module, multi-modal learning-enabled Cyber-Physical Systems (CPS). Such industry-relevant CPS integrate various functionalities like perception, planning, and prediction and utilize a range of sensors including cameras, Lidar, and radar~\cite{lou2022testing,prakash2021multi}.

%There has been a surge in research focusing on the formal verification of machine learning models using 
%geometric reachability (NNV star set~\cite{tran2020verification}), mixed-interger programming feasibility e(Sherlock~\cite{dutta2019sherlock}), SMT solver (Reluplex~\cite{katz2017reluplex}) and model-free optimization (Branch and Bound~\cite{bunel2018unified}).
%~\cite{katz2017reluplex,ehlers2017formal,zhang2018efficient,katz2019marabou}. 
%This line of research primarily targets the robustness and safety of the models themselves. However, a common limitation in these studies is the treatment of robustness as a predefined geometric input space, wherein a search is conducted to identify a radius where the model's predictions remain stable or bounded by linear constraints. In recent neural network verification competitions~\cite{bak2021second}, efforts have been made to examine properties like the prevention of aircraft collisions~\cite{owen2019acas}. 
%However, these initiatives frequently fall short in aligning with formal specifications essential for system safety, such as Signal Temporal Logic~\cite{donze2010robust}. Moreover, the target systems—often consisting of single models—are overly simplistic in both their input spaces and architectural complexities, especially when compared to industry-scale, multi-module, multi-modal learning-enabled CPS including perception, planning and prediction with cameras, Lidar and radar sensors~\cite{lou2022testing,prakash2021multi}.

Recent research in the system domain has explored in-situ reasoning for closed-loop systems. In one example~\cite{tuncali2018reasoning}, barrier certificates serve as differentiable invariant functions that, in conjunction with a non-linear SMT solver, provide safety guarantees. These guarantees state that from a set of possible initial conditions, a set of unsafe states will not be reached. However, identifying these states remains challenging, and questions about the scalability and applicability of this approach to multi-module learning-enabled systems remain unanswered. 

Simultaneously, the testing landscape for learning-enabled CPS has seen considerable research activity. One primary focus area has been the verification of system properties, specifically concerning accuracy~\cite{deng2022declarative} and safety~\cite{tian2022mosat,li2020av}. Parallel to this, another research direction has honed in on evaluating system robustness. This includes metrics like resilience to data corruption~\cite{tian2018deeptest}, adversarial robustness~\cite{deng2020analysis}, and the system's ability to generalize when faced with shifts in data distribution~\cite{cai2020real}.
%Recent research has delved extensively into the testing of various facets of learning-enabled CPS. One prominent direction of this research is dedicated to verifying the accuracy~\cite{deng2022declarative} and safety~\cite{tian2022mosat,li2020av} properties inherent to these systems. Concurrently, another research trajectory is centered on evaluating the robustness of such systems, taking into account factors like corruption robustness~\cite{tian2018deeptest}, adversarial resilience~\cite{deng2020analysis}, and generalization under distribution shifts~\cite{cai2020real}. 
However, a significant portion of the current testing methodologies employs fitness functions that encompass multiple objectives or coverage metrics. These approaches lack any concrete formal guarantees concerning formal specifications. While there are recent studies \cite{sun2022lawbreaker,zhou2023specification} that incorporate formal specifications, specifically in the form of STL, these specifications tend to be narrowly tailored to specific manually defined scenarios, such as lane changes or navigating intersections. As a result, they fall short in offering a comprehensive safety guarantee (e.g., ensuring no crashes). Furthermore, the test cases derived from these methodologies don't provide a stringent guarantee regarding the extent to which the specified properties are met. From an industrial perspective, particularly in sectors deploying learning-enabled CPS, existing testing methodologies are largely probabilistic in nature. What the industry is increasingly calling for are tangible formal guarantees. For example, in the context of self-driving cars, while it may be unrealistic to claim that an autonomous vehicle will never be involved in an accident, there should be a robust safety assurance that the vehicle will not be a contributing factor to the causation of any accident~\cite{shalev2017formal}.

Certainly, testing remains the most pragmatically adopted method for ensuring the reliability and safety of systems in industry, particularly for complex learning-enabled CPS. If testing methodologies can be designed to rigorously evaluate systems against formal specifications, then they would offer a meaningful form of formal guarantee. This approach would occupy a middle ground between two existing paradigms: model checking and runtime verification. On one end, formal verification (model checking~\cite{kochdumper2023fully}) aims to exhaustively verify properties against all possible behaviors of the system, a process that is often computationally infeasible for complex, large-scale systems like learning-enabled CPS and  more critically, verifying individual learning-enabled components (LEC) and attempting
to compose guarantees of individual components
into system-level guarantees is not available~\cite{seshia2017compositional}. On the other end, runtime verification~\cite{zapridou2020runtime} monitors properties against observed runtime traces, offering no guarantees about unobserved behaviors and often requiring a large number of samples for confidence. Incorporating formal specifications into a test-based methodology could offer a more feasible yet comprehensive alternative. It would not only be more aligned with industrial practices but would also be more computationally tractable than exhaustive model checking, while still offering broader assurances than runtime verification.

In this paper, we outline a research roadmap to enhance testing methodologies for learning-enabled Cyber-Physical Systems. Leveraging large-language models, we aim to generate rigorous test cases, extract formal specifications from this test data, and then test against these specifications. This approach offers a more practical yet robust alternative to existing methods, providing a form of formal guarantee that aligns with industrial needs.


%Linear-time temporal logic guided greybox fuzzing
%Given a linear-time temporal logic (LTL) property $\phi$, a B\"uchi automata $\mathrm{A}\neg\phi$ can be constructed which accepte the violation of the property $\phi$.  But the approach requires to identify program locations where the atomic propositions in the LTL property may be affected, which is not possible in learning-based CPS where corresponding locations do not exist (e.g., speed control resides in multiple neural networks from perception, prediction to planning for self-drving cars).


%The amount of data
%required to guarantee a probability of $10^(-9)$ fatality per hour of driving is proportional to its inverse, $10^9$ hours of data
%(see details in the sequel), which is roughly in the order of thirty billion miles~\cite{shalev2017formal}. 



%1. Do not hit someone from behind.
%2. Do not cut-in recklessly.
%3. Right-of-way is given, not taken.
%4. Be careful of areas with limited visibility
%5. If you can avoid an accident without causing another one, you must do it~\cite{shalev2017formal}


%verification where one checks whether all system behaviors satisfy
%', LTL is also used for lightweight verification (monitoring, runtime verification [5])
%where the satisfaction of a formula by one or more individual behaviors is checked.
%For both uses, monitoring and verification alike, we point out three fundamental features
%of this framework, the first two related to the nature of the systems and behaviors
%considered while the third is related to the very notion of property and logical truth.
%1. Discrete qualitative time: behaviors are defined as sequences of states or events,
%which are often interpreted in a purely qualitative manner, that is, without considering
%the metric distance between subsequent time instances;
%2. Discrete state space: the sequences are defined over %discrete and often finite domains
%emphasizing control rather than data;
%3. Yes/No answer: the satisfaction of a temporal formula by a behavior is considered
%as membership in a set, with no quantitative degree of satisfaction. They present an efficeint dense-time algorithm for computing both Space (predicate over signals) and time (duration of events) robustness for piecewise-linear signals~\cite{donze2010robust}.

%Fainekos and Pappas~\cite{fainekos2009robustness} define the notion of robustness degree
%as a real number associated with a property-behavior pair, based on, roughly speaking,
%the distance between the behavior and the (boundary of) the set of all behaviors that satisfy
%the property. This measure is more positive when the behavior is deeper inside the
%set of satisfying behaviors and more negative the further is the behavior outside that set. Behavior-oriented approach to modify signal to satisfy or violate the property.

%\begin{bmatrix}
%\frac{\partial f}{\partial x_1} \\
%\frac{\partial f}{\partial x_2} \\
%\vdots \\
%\frac{\partial f}{\partial x_n}
%\end{bmatrix} 

%\begin{bmatrix}
%\frac{\partial f_1}{\partial x_1} & \frac{\partial f_1}%{\partial x_2} & \dots & \frac{\partial f_1}{\partial x_n} \\
%\frac{\partial f_2}{\partial x_1} & \dots & \dots & \frac{\partial f_2}{\partial x_n} \\
%\vdots & \vdots & \ddots & \vdots \\
%\frac{\partial f_m}{\partial x_1} & \dots & \dots & \frac{\partial f_m}{\partial x_n}
%\end{bmatrix}
